Coherent differentiation with a monoid of degrees: derivatives, Taylor expansion, finite differences...

Coherent differentiation has been introduced a few years ago as a refinement of the (categorical semantics of the) differential lambda-calculus and of differential linear logic, compatible with the determinism of computation, and hence in categories where addition of morphisms in the hom-sets is only partially defined. In this setting differentiation is implemented by a kind of ''tangent functor'', with the difference that it maps an object to its object of summable tuples rather to a tangent bundle. In our earlier work, these tuples were pairs in the case of simple differentiation, and families indexed by integers when dealing with Taylor expansion and the Fa{\`a} di Bruno formula. We push this idea further, considering now tuples indexed by an arbitrary commutative partial monoid satisfying a nonnegativity condition. The monoid structure on these indices plays a crucial role in the definition of the ''differential'' calculus associated with this ''tangent functor''. In that way, and without changing the general categorical infrastructure of coherent differentiation, this theory accommodates new notions of ''differentiation'' of which we describe several instances. Among many others, such notions include various forms of finite differences as well as Taylor expansion truncated at any fixed degree, and finite Taylor expansion of a fixed finite degree with a remainder.

==> mainnot.tex <==

% Setup double \llangle and \rrangle
\makeatletter
\DeclareFontFamily{OMX}{MnSymbolE}{}
\DeclareSymbolFont{MnLargeSymbols}{OMX}{MnSymbolE}{m}{n}
\SetSymbolFont{MnLargeSymbols}{bold}{OMX}{MnSymbolE}{b}{n}
\DeclareFontShape{OMX}{MnSymbolE}{m}{n}{
    <-6>  MnSymbolE5
   <6-7>  MnSymbolE6
   <7-8>  MnSymbolE7
   <8-9>  MnSymbolE8
   <9-10> MnSymbolE9
  <10-12> MnSymbolE10
  <12->   MnSymbolE12
}{}
\DeclareFontShape{OMX}{MnSymbolE}{b}{n}{
    <-6>  MnSymbolE-Bold5
   <6-7>  MnSymbolE-Bold6
   <7-8>  MnSymbolE-Bold7
   <8-9>  MnSymbolE-Bold8
   <9-10> MnSymbolE-Bold9
  <10-12> MnSymbolE-Bold10
  <12->   MnSymbolE-Bold12
}{}

\let\llangle\@undefined
\let\rrangle\@undefined
\DeclareMathDelimiter{\llangle}{\mathopen}%
                     {MnLargeSymbols}{'164}{MnLargeSymbols}{'164}
\DeclareMathDelimiter{\rrangle}{\mathclose}%
                     {MnLargeSymbols}{'171}{MnLargeSymbols}{'171}
\makeatother

\makeatletter
\newcommand{\labeltext}[2]{%
  \@bsphack
  \csname phantomsection\endcsname % in case hyperref is used
  \def\@currentlabel{#1}{\label{#2}}%
  \@esphack
}
\makeatother



\newcommand\Redparagraph[1]{\paragraph{#1~:}}

\makeatletter
\newcommand*{\inlineeq}[2][]{%
  \begingroup
    % Put \refstepcounter at the beginning, because
    % package `hyperref' sets the anchor here.
    \refstepcounter{equation}%
    \ifx\\#1\\%
    \else
      \label{#1}%
    \fi
    % prevent line breaks inside equation
    \relpenalty=10000 %
    \binoppenalty=10000 %
    \ensuremath{%
      % \displaystyle % larger fractions, ...
      #2%
    }%
    ~\@eqnnum
  \endgroup
}
\makeatother

\theoremstyle{definition}
%\newtheorem{example}{Example}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{remark}[definition]{Remark}
\crefname{remark}{Remark}{Remarks}
\newtheorem{example}[definition]{$\blacktriangleright$ \ Example}
\crefname{example}{Example}{Examples}

\theoremstyle{plain}
\newtheorem{lemma}[definition]{Lemma}
\crefname{lemma}{Lemma}{Lemmas}
\newtheorem{theorem}[definition]{Theorem}
\newtheorem{corollary}[definition]{Corollary}
\newtheorem{proposition}[definition]{Proposition}



\newenvironment{Example}
  {\begin{example}} 
  {\hphantom{0em}\hfill$\blacktriangleleft$ 
  \end{example}}
   

\newenvironment{Axicond}[1]
{\smallbreak\noindent{#1}\,}
{\smallbreak}

\newcommand\Ie{\textsl{i.e.}}
\newcommand\Etc{\textsl{etc.}}

% \let\oldequation\equation
% \let\oldendequation\endequation

% \renewenvironment{equation}
%   {\linenomathNonumbers\oldequation}
%   {\oldendequation\endlinenomath}

% \renewenvironment{align*}
%   {\begin{linenomath}\begin{align*}}
%   {\end{align*}\end{linenomath}}

\newcommand\Insbreak{\bigbreak\bigbreak\bigbreak\bigbreak\bigbreak\bigbreak
\noindent\hrule
\bigbreak\noindent\hrule
\bigbreak}


\newcommand{\qqbox}[1]{\quad\hbox{{#1}}\quad}
\newcommand{\qbox}[1]{\quad\hbox{{#1}}}
\newcommand{\bbbox}[1]{\ \hbox{{#1}}\ }
\newcommand{\bbox}[1]{\ \hbox{{#1}}}

% \newtheorem*{lemma*}{Lemma}
% \newtheorem*{proposition*}{Proposition}
\newtheorem{convention}[definition]{Convention}


% \makeatletter%
% \renewcommand\subsubsection{%
% \@startsection{subsubsection}{3}{0mm}{\baselineskip}{-1em}%
% {\normalfont\bfseries}}
% \makeatother
% \renewcommand\paragraph{\subsubsection}


\newcommand\rulename[1]{\smallbreak\noindent\textbf{#1}:}

\newcommand\Proofbreak{\smallbreak}

\newcommand\Proofcase{\smallbreak\noindent$\blacktriangleright$\ }

\def\bull{\vrule height.9ex width.8ex depth-.1ex}

\newcommand{\proofitem}[1]{\paragraph*{\mdseries\textit{#1}}}

\newcommand{\Beginproof}{\proofitem{Proof.}}
\newcommand{\Endproof}{
  \ifmmode % if math mode, assume display: omit penalty etc.
  \else \leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
  \fi
  \quad\hbox{$\Box$}
  \par\medskip}

\newcommand\Condl[1]{\label{cond:#1}}
\newcommand\Condr[1]{(\ref{cond:#1})}

\newcommand\Eqref[1]{(\ref{#1})}

\newcommand\Eg{\textsl{e.g.}}


% \newenvironment{remark}%
% {\smallbreak\noindent{\textit{Remark\/}: }\nobreak}%
% {\smallbreak}

\renewcommand{\phi}{\varphi}
\renewcommand\epsilon{\varepsilon}
\renewcommand\sharp{\#}

\newcommand{\Iff}{\quad\hbox{iff}\quad}
\newcommand{\Ifsimple}{\quad\hbox{if}\quad}
\newcommand{\Implies}{\Rightarrow}
\newcommand{\Implsymbol}{\Rightarrow}
\newcommand\Equiv{\Leftrightarrow}
\newcommand{\St}{\mid}

% \newcommand\Carrier[1]{\lfloor{#1}\rfloor}
\newcommand\Carrier[1]{{|#1|}}

\newcommand{\Ro}{\circ}
\newcommand{\Inf}{\bigwedge}
\newcommand{\Infi}{\wedge}
\newcommand{\Sup}{\bigvee}
\newcommand{\Supi}{\vee}

%\newcommand{\Filled}[1]{\Myleft|{#1}\Myright|}

\newcommand{\arrow}{\rightarrow}
\newcommand{\Bott}{{\mathord{\perp}}}
\newcommand{\Sbot}{{\mathord{\perp}}}
\newcommand{\Top}{\top}
%\newcommand{\Zero}{0}

\newcommand\Seqempty{\Tuple{}}

\newcommand\cA{\mathcal{A}}
\newcommand\cB{\mathcal{B}}
\newcommand\cC{\mathcal{C}}
\newcommand\cD{\mathcal{D}}
\newcommand\cE{\mathcal{E}}
\newcommand\cF{\mathcal{F}}
\newcommand\cG{\mathcal{G}}
\newcommand\cH{\mathcal{H}}
\newcommand\cI{\mathcal{I}}
\newcommand\cJ{\mathcal{J}}
\newcommand\cK{\mathcal{K}}
\newcommand\cL{\mathcal{L}}
\newcommand\cM{\mathcal{M}}
\newcommand\cN{\mathcal{N}}
\newcommand\cO{\mathcal{O}}
\newcommand\cP{\mathcal{P}}
\newcommand\cQ{\mathcal{Q}}
\newcommand\cR{\mathcal{R}}
\newcommand\cS{\mathcal{S}}
\newcommand\cT{\mathcal{T}}
\newcommand\cU{\mathcal{U}}
\newcommand\cV{\mathcal{V}}
\newcommand\cW{\mathcal{W}}
\newcommand\cX{\mathcal{X}}
\newcommand\cY{\mathcal{Y}}
\newcommand\cZ{\mathcal{Z}}

\newcommand\CAT{\mathbf{Cat}}


\newcommand\Fini{{\mathrm{fin}}}



\def\frownsmile{%
\mathrel{\vbox{\hbox{${\frown}$}\vspace{-2ex}\hbox{${\smile}$}\vspace{-.5ex}}}}
\def\smilefrown{%
\mathrel{\vbox{\hbox{${\smile}$}\vspace{-2ex}\hbox{${\frown}$}\vspace{-.5ex}}}}

\newcommand\Part[1]{{\mathcal P}\left({#1}\right)}
\newcommand\Parti[1]{{\mathcal I}({#1})}

\newcommand\Union{\bigcup}

\newcommand{\Linarrow}{\multimap}

\def\frownsmile{%
\mathrel{\vbox{\hbox{${\frown}$}\vspace{-2ex}\hbox{${\smile}$}\vspace{-.5ex}}}}
\def\smilefrown{%
\mathrel{\vbox{\hbox{${\smile}$}\vspace{-2ex}\hbox{${\frown}$}\vspace{-.5ex}}}}

\newcommand\CScoh[3]{{#2}\mathrel{\frownsmile_{{#1}}}{#3}}
\newcommand\CScohs[3]{{#2}\mathrel{{\frown}_{#1}}{#3}}
\newcommand\CScohstr[3]{\CScohs{#1}{#2}{#3}}
\newcommand\CSincoh[3]{{#2}\mathrel{\smilefrown_{{#1}}}{#3}}
\newcommand\CSincohs[3]{{#2}\mathrel{{\smile}_{#1}}{#3}}
\newcommand\CSeq[3]{{#2}\mathrel{{=}_{#1}}{#3}}

\newcommand\Myleft{}
\newcommand\Myright{}

\newcommand\Web[1]{\Myleft|{#1}\Myright|}
%\newcommand\Supp[1]{\Myleft|{#1}\Myright|}
\newcommand\Suppsymb{\operatorname{\mathsf{supp}}}
\newcommand\Supp[1]{\operatorname{\mathsf{supp}}({#1})}
\newcommand\Suppms[1]{\operatorname{\mathsf{set}}({#1})}
%\newcommand\Suppms[1]{\underline{#1}}

\newcommand\Emptymset{[\,]}
\newcommand\Mset[1]{[{#1}]}
%\newcommand\Sset[1]{\langle{#1}\rangle}
\newcommand\Sset[1]{({#1})}


\newcommand\MonP{P}
\newcommand\MonPZ{\MonP_0}

\newcommand\Cl[1]{\mbox{\textrm{Cl}}({#1})}
\newcommand\ClP[1]{\mbox{\textrm{Cl}}_{\MonP}({#1})}

\newcommand\Star{\star}
\newcommand\CohName{\mathbf{Coh}}
\newcommand\NCohName{\mathbf{NCoh}}
\newcommand\COH{\CohName}
\newcommand\NCOH{\NCohName}
\newcommand\COHR[2]{\CohName(#1,#2)}

\newcommand\Par[2]{{#1}\mathrel{\IPar}{#2}}
\newcommand\Parp[2]{\left({#1}\mathrel{\IPar}{#2}\right)}
\newcommand\ITens{\mathrel\otimes}
\newcommand\Tens[2]{{#1}\ITens{#2}}
\newcommand\Comma[2]{{#1},{#2}}
\newcommand\Tensp[2]{({#1}\ITens{#2})}
\newcommand\Tenspb[2]{\big({#1}\ITens{#2}\big)}
\newcommand\TenspB[2]{\Big({#1}\ITens{#2}\Big)}
\newcommand\IWith{\mathrel{\&}}
\newcommand\With[2]{{#1}\IWith{#2}}
\newcommand\Withe[2]{{#1}\IWith^\Klsymb{#2}}
\newcommand\Withep[2]{\left({#1}\IWith^\Klsymb{#2}\right)}
\newcommand\Withp[2]{\left({#1}\IWith{#2}\right)}
\newcommand\IPlus{\oplus}
\newcommand\Plus[2]{{#1}\IPlus{#2}}
%\newcommand\ILfun{\multimap}
%\newcommand\Lfun[2]{{#1}\ILfun{#2}}
\newcommand\Orth[2][]{#2^{\mathord\perp_{#1}}}
\newcommand\Orthp[2][]{(#2)^{\Bot_{#1}}}

\newcommand\Klsymb{\mathsf K}

\newcommand\Bwith{\mathop{\&}}
\newcommand\Bwithe{\mathop{\&^{\Klsymb}}}
\newcommand\Bplus{\mathop\oplus}
\newcommand\Bunion{\mathop\cup}

\newcommand\Scal[2]{\langle{#1}\mid{#2}\rangle}

%\newcommand\App[2]{{#1}[{#2}]}

\newcommand\Pair[2]{\langle{#1},{#2}\rangle}

%\newcommand\Inj{\lambda}
\newcommand\Inj[1]{\overline\pi_{#1}}

\newcommand\GlobalIndex{I}
\newcommand\Index{\GlobalIndex}
\newcommand\Relbot{\Bot_\Index}
%\newcommand\Relbot{\Bot}
\newcommand\MonPZI{{\MonPZ}^\Index}
\newcommand\ClPI[1]{{\ClP{{#1}}}^\Index}
\newcommand\WebI[1]{\Web{#1}^\Index}


%\newcommand\Bar{\vec}
%\renewcommand\Bar{}
\newcommand\Scalb[2]{\Scal{\Bar{#1}}{\Bar{#2}}}

\newcommand\Ortho[2]{{#1}\mathrel{\bot}{#2}}
\newcommand\Orthob[2]{\Bar{#1}\mathrel{\bot}\Bar{#2}}

\newcommand\Biorth[1]{#1^{\bot\bot}}
\newcommand\Biorthp[3]{{#1}^{\Bot_{#2}\Bot_{#3}}}
\newcommand\Triorth[1]{{#1}^{\bot\bot\bot}}
\newcommand\Triorthp[4]{{#1}^{\Bot_{#2}\Bot_{#3}\Bot_{#4}}}

\newcommand\Relpretens[2]{\cR_{#1}\bar\ITens\cR_{#2}}
\newcommand\Relpreplus[2]{\cR_{#1}\bar\IPlus\cR_{#2}}

%\newcommand\Rel[1]{\cR_{#1}}

\newcommand\RelP[1]{\widetilde{#1}}

\newcommand\Eqw[2]{\delta({#1},{#2})}
\newcommand\Eqwb[2]{\Eqw{\Bar{#1}}{\Bar{#2}}}

\newcommand\PFacts[1]{\cF({#1})}
%\newcommand\Facts{\cF(\MonPZI)}

\newcommand\Facts{\cF(\MonPZI)}


\newcommand\RelL[1]{\overline{#1}}

\newcommand\PRel[1]{R_{#1}}

\newcommand\PFamb[2]{[\Bar{#1},\Bar{#2}]}

\newcommand\Fplus[2]{\Bar{#1}+\Bar{#2}}

\newcommand\Char[1]{\epsilon_{#1}}

\newcommand\Fproj[2]{\pi_{#1}(\Bar{#2})}

\newcommand\One{1}


\newcommand\Pbot[1]{\Bot_{#1}}
\newcommand\PBot[1]{\Bot_{#1}}
\newcommand\PRBot[1]{\Bot_{#1}}
\newcommand\PROne[1]{1_{#1}}

\newcommand\Pproj[1]{\pi_{#1}}

\newcommand\Zext[1]{\zeta_{\Bar{#1}}}
\newcommand\Aext[1]{\bar\zeta_{\Bar{#1}}}

\newcommand\Mall{\hbox{\textsf{MALL}}}
\newcommand\RMall{\Mall(\Index)}
\newcommand\RMallr[1]{\Mall({#1})}
\newcommand\FDom[1]{d({#1})}

% constantes relativisees
\newcommand\RBot[1]{\Bot_{#1}}
\newcommand\ROne[1]{\One_{#1}}

% sequent
\newcommand\Seq[1]{\vdash{#1}}

% sequent relativise a un ensemble
\newcommand\RSeq[2]{\vdash_{#1}{#2}}

% restriction d'une formule de MALL(J)
\newcommand\Restr[2]{{#1}|_{#2}}
\newcommand\FRestr[2]{{#1}|_{#2}}

% semantique d'une formule et d'une preuve
\newcommand\FSem[1]{{#1}^{*}}
\newcommand\PSem[1]{{#1}^{*}}

% formule de MALL(J) associee a une famille de points de la trame
\newcommand\FFamb[2]{{#1}\langle\Bar{#2}\rangle}

\newcommand\Premskip{\hskip1cm}
%\newcommand\Forg[1]{\FRestr{#1}\emptyset}
\newcommand\Forg[1]{\underline{#1}}

\newcommand\Phase[1]{{#1}^\bullet}

\newcommand\Punit[1]{1^{#1}}

\newcommand\Reg[1]{R_{#1}}

\newcommand\Cont[1]{{#1}^\circ}

\newcommand\Neutral{e}
\newcommand\RNeutral[1]{\Neutral_{#1}}

\newcommand\POne{1}

\newcommand\relstack[2]{\underset{#2}{#1}}
\newcommand\RPlus[4]{{#3}\relstack\IPlus{{#1},{#2}}{#4}}
\newcommand\RWith[4]{{#3}\relstack\IWith{{#1},{#2}}{#4}}

\newcommand\PReq[1]{=_{#1}}

\newcommand\Fam[2]{\hbox{\textrm{Fam}}_{#1}(#2)}
\newcommand\Famfunc[1]{\hbox{\textrm{Fam}}_{#1}}

\newcommand\Pval[1]{\rho_{#1}}

\newcommand\Fcoh{\mathsf C}
\newcommand\Fincoh{\overline\Fcoh}
\newcommand\Feq{\mathsf E}

\newcommand\RZero{\Zero}
\newcommand\RTop{\Top}
\newcommand\EmptyFam{\emptyset}
\newcommand\Partial[1]{\Omega_{#1}}

\newcommand\PMall{\hbox{\textsf{MALL}}_\Omega}
\newcommand\PRMall{\Mall_\Omega(\Index)}
\newcommand\Homo[1]{H(#1)}
\newcommand\RProd[2]{\Lambda_{#1}{({#2})}}
\newcommand\FProd[1]{\widetilde{#1}}

\newcommand\CltoPCl[1]{{#1}^P}

\newcommand\Partfin[1]{{\cP_\Fini}({#1})}



\newcommand\RLL{\LL(\Index)}
\newcommand\RLLP{\LL^+(\Index)}
\newcommand\RLLext{\LL^\mathrm{ext}(\Index)}

\newcommand\IExcl{{\mathord{!}}}
\newcommand\IInt{{\mathord{?}}}

\newcommand\RExcl[1]{\IExcl_{#1}}
\newcommand\RInt[1]{\IInt_{#1}}


\newcommand\Fempty[1]{0_{#1}}

\newcommand\FAct[1]{{#1}_*}

\newcommand\Noindex[1]{\langle{#1}\rangle}

\newcommand\Card[1]{\#{#1}}
\newcommand\Multi[1]{\mathsf m({#1})}

\newcommand\FamRestr[2]{{#1}|_{#2}}

\newcommand\Pact[1]{{#1}_*}

\newcommand\Pinj[1]{\zeta_{#1}}

\newcommand\Locun[1]{1^J}

\newcommand\Isom\simeq
\newcommand\Webisom{\simeq_{\mathsf w}}

\newcommand\FGraph[1]{\mathsf{g}({#1})}
\newcommand\GPFact[1]{\mathsf f_0({#1})}
\newcommand\GFact[1]{\mathsf f({#1})}

% \newcommand\NUCS{non-uniform coherence space}
% \newcommand\NUCSb{non-uniform coherence space }
% \newcommand\NUCSs{non-uniform coherence spaces}
% \newcommand\NUCSsb{non-uniform coherence spaces }
\newcommand\NUCS{\mathbf{nCoh}}

\newcommand\Comp{\mathrel\circ}
\newcommand\Compfun{\,}

\newcommand\Funinv[1]{{#1}^{-1}}

\newcommand\Reindex[1]{{#1}^*}

\newcommand\Locbot[1]{\Bot({#1})}
\newcommand\Locone[1]{1({#1})}
\newcommand\LocBot{\Locbot}
\newcommand\LocOne{\Locone}

\newcommand\INJ[1]{\mathcal I({#1})}
\newcommand\COHP[1]{\mathcal C({#1})}
\newcommand\FuncFam[1]{\mathrm{Fam}_{#1}}
\newcommand\SET{\mathbf{Set}}
\newcommand\PSET{\mathbf{Set}_0}
\newcommand\Locmod[2]{{#1}({#2})}
\newcommand\FuncPhase[1]{\mathcal{F}_{#1}}
\newcommand\Trans[2][]{{\widehat{#2}}_{#1}}
\newcommand\Useful[1]{\Web{#1}_{\mathrm u}}

\newcommand\Limpl[2]{{#1}\Linarrow{#2}}
\newcommand\Limplp[2]{\left({#1}\Linarrow{#2}\right)}

\newcommand\ConstFam[2]{{#1}^{#2}}

\newcommand\Projtr[1]{{\mathsf{pr}}^{#1}}
\newcommand\Injtr[1]{{\mathsf{in}}^{#1}}

\newcommand\Center[1]{\mathcal C({#1})}

\newcommand\Derel[1]{\mathrm{d}_{#1}}

\newcommand\Mspace[2]{{#2}^*_{#1}}

\newcommand\CStoMS[1]{{#1}^+}
\newcommand\MStoCS[1]{{#1}^-}

\newcommand\PhaseCoh[1]{{\mathbf{Coh}}_{#1}}

\newcommand\Nat{{\mathbb{N}}}
\newcommand\Relint{{\mathbb{Z}}}
\newcommand\Natnz{{\Nat^+}}

\newcommand\Rien{\Omega}

\newcommand\DenEq[2]{{#1}\sim{#2}}

\newcommand\VMon[2]{\langle{#1},{#2}\rangle}
\newcommand\VMonc[3]{\langle{#1},{#2},{#3}\rangle}

%\newcommand\Multind[1]{\begin{substack}#1\end{substack}}
%\newcommand\Biind[2]{\scriptstyle{#1}\atop\scriptstyle{#2}}
\newcommand\Biind[2]{\genfrac{}{}{0pt}{1}{#1}{#2}}

\newcommand\Adapt[1]{\cA_{#1}}

\newcommand\Rllp[1]{\widetilde{#1}}

\newcommand\Emptyfun[1]{0_{#1}}

\newcommand\Multisetfin[1]{\mathcal{M}_{\mathrm{fin}}({#1})}

\newcommand\Myparag[1]{\noindent\textbf{#1.}\ }

\newcommand\Webinf[1]{\Web{#1}_\infty}
%\newcommand\Fin[1]{\mathrm{F}({#1})}
\newcommand\Fin[1]{\mathsf{F}({#1})}
%\newcommand\Fin[1]{\mathcal{F}({#1})}
%\newcommand\Fin[1]{\Phi({#1})}

\newcommand\Phasefin{\mathbb{F}}

\newcommand\Fspace[1]{\mathrm f{#1}}
\newcommand\Space[1]{\mathrm m{#1}}


\newcommand\Ssupp[1]{\Supp{#1}}

\newcommand\FIN{\mathbf{Fin}}
\newcommand\FINH[2]{\FIN({#1},{#2})}
\newcommand\FINF[1]{\FIN[{#1}]}
\newcommand\SETINJ{\mathbf{Inj}}
\newcommand\EMB{\FIN_{\mathrm e}}

\newcommand\SNat{\mathsf N}
\newcommand\Snat{\mathsf N}
\newcommand\Snatcoh{\mathsf N^\NUCS}

\newcommand\Iter[1]{\mathsf{It}_{#1}}
\newcommand\Piter[2]{\Iter{#1}^{(#2)}}
\newcommand\Case[1]{\mathsf{Case}_{#1}}
% \newcommand\Fix[1]{\mathsf{Y}_{#1}}
\newcommand\Pfix[2]{\mathsf{Y}_{#1}^{(#2)}}
\newcommand\Ifthenelse[3]{\mathtt{if}\,{#1}\,\mathtt{then}\,{#2}\,%
\mathtt{else}\,{#3}}

\newcommand\Ptrace[1]{\|{#1}\|}
\newcommand\Enat[1]{\overline{#1}}
\newcommand\FA[1]{\forall{#1}}
% \newcommand\Trcl[2]{\langle {#1},{#2}\rangle}
\newcommand\Faproj[1]{\epsilon^{#1}}
\newcommand\Faintro[3]{\Lambda^{{#1},{#2}}({#3})}

\newcommand\Bool{\mathbf{Bool}}
\newcommand\True{\mathbf t}
\newcommand\False{\mathbf f}


\newcommand\Tarrow{\arrow}
\newcommand\Diffsymb{\mathsf D}
\newcommand\Diffapp[2]{\mathsf D{#1}\cdot{#2}}
\newcommand\Diff[3]{\mathrm D_{#1}{#2}\cdot{#3}}
\newcommand\Diffexp[4]{\mathrm D_{#1}^{#2}{#3}\cdot{#4}}
\newcommand\Diffvar[3]{\mathrm D_{#1}{#2}\cdot{#3}}
\newcommand\Diffterm[3]{\mathrm D_{#1}{#2}\cdot{#3}}
\newcommand\Zero{0}
\newcommand\App[2]{\mathsf{ap}({#1}, {#2})}
\newcommand\Appb[2]{\big({#1}\big){#2}}
\newcommand\AppB[2]{\Big({#1}\Big){#2}}
\newcommand\Apppref[1]{\left({#1}\right)}
\newcommand\Appp[3]{\left({#1}\right){#2}\,{#3}}
\newcommand\Abs[2]{\lambda{#1}\,{#2}}
\newcommand\Abst[3]{\lambda#1^{#2}\,{#3}}
%\newcommand\Diffp[3]{{\partial{#1}\over\partial{#2}}\cdot u}
\newcommand\Diffp[3]{\frac{\partial{#1}}{\partial{#2}}\cdot{#3}}
\newcommand\Diffpev[4]{\frac{\partial{#1}}{\partial{#2}}(#3)\cdot{#4}}
\newcommand\Diffr[3]{d{\partial{#1}}{d{#2}}\cdot{#3}}
\newcommand\Derp[3]{\frac{\partial{#1}}{\partial{#2}}\cdot{#3}}
\newcommand\Derd[3]{\frac{d{#1}}{d{#2}}\cdot{#3}}
\newcommand\Derdn[4]{\frac{d^{#1}{#2}}{d{#3}^{#1}}\cdot{#4}}
\newcommand\Derdev[4]{\frac{d{#1}}{d{#2}}(#3)\cdot{#4}}
\newcommand\Derplist[4]{%
\frac{\partial^{#4}{#1}}{\partial#2_1\cdots\partial#2_{#4}}%
\cdot\left(#3_1,\dots,#3_{#4}\right)}
\newcommand\Derplistexpl[6]{%
\frac{\partial^{#6}{#1}}{\partial{#2}\cdots\partial{#3}}%
\cdot\left({#4},\dots,{#5}\right)}
\newcommand\Derpmult[4]{%
\frac{\partial^{#4}{#1}}{\partial{#2}^{#4}}%
\cdot\left(#3_1,\dots,#3_{#4}\right)}
\newcommand\Derpm[4]{%
\frac{\partial^{#4}{#1}}{\partial{#2}^{#4}}%
\cdot\left({#3}\right)}
\newcommand\Derpmultgros[4]{%
\frac{\partial^{#4}}{\partial{#2}^{#4}}\left({#1}\right)%
\cdot\left(#3_1,\dots,#3_{#4}\right)}
\newcommand\Derpmultbis[4]{%
\frac{\partial^{#4}{#1}}{\partial{#2}^{#4}}%
\cdot{#3}}
\newcommand\Derpmultbisgros[4]{%
\frac{\partial^{#4}}{\partial{#2}^{#4}}\left({#1}\right)%
\cdot{#3}}
\newcommand\Derppar[3]{\left(\Derp{#1}{#2}{#3}\right)}
\newcommand\Derpgros[3]{\frac{\partial}{\partial{#2}}\Bigl({#1}\Bigr)%
\cdot{#3}}
\newcommand\Derpdeux[4]{\frac{\partial^2{#1}}{\partial{#2}\partial{#3}}%
\cdot{#4}}
\newcommand\Derpdeuxbis[5]{\frac{\partial^{#5}{#1}}{\partial{#2}\partial{#3}}%
\cdot{#4}}
\newcommand\Diffpv[3]{\frac{\partial}{\partial{#2}}{#1}\cdot{#3}}
\newcommand\Diffpd[5]{\frac{\partial^2{#1}}{\partial{#2}\partial{#3}}%
\cdot\left({#4},{#5}\right)}

\newcommand\Paragraph[1]{\smallbreak\noindent\textbf{#1}}
\newcommand\Parag[1]{\S\ref{#1}}

%\newcommand\Redone{\mathrel{\beta^1_{\mathrm D}}}
\newcommand\Redamone{\mathrel{\beta^{0,1}}}
\newcommand\Redonecan{\mathrel{{\bar\beta}^1_{\mathrm D}}}
%\newcommand\Red{\mathrel{\beta}}
\newcommand\Redpar{\mathrel{\rho}}
\newcommand\Redparcan{\mathrel{\bar\rho}}

\newcommand\Sat[1]{#1^*}

\newcommand\Can[1]{\left\langle{#1}\right\rangle}
\newcommand\Candiff[3]{\Delta_{#1}{#2}\cdot{#3}}

%\newcommand\Eq{\simeq}
\newcommand\Eq{\simeq}

\newcommand\List[3]{#1_{#2},\dots,#1_{#3}}
\newcommand\Listbis[3]{#1_{#2}\dots #1_{#3}}
\newcommand\Listter[3]{#1_{#2}\cdots #1_{#3}}
\newcommand\Listc[4]{{#1}_{#2},\dots,{#4},\dots,{#1}_{#3}}
\newcommand\Listbisc[4]{{#1}_{#2}\dots{#4}\dots{#1}_{#3}}
\newcommand\Absent[1]{\widehat{#1}}
\newcommand\Kronecker[2]{\boldsymbol\delta_{{#1},{#2}}}

\newcommand\Eqindent{\quad}

\newcommand\Subst[3]{{#1}\left[{#2}/{#3}\right]}
\newcommand\Substv[3]{{#1}\left[{#2\,}/{#3}\right]}
\newcommand\Substz[2]{{#1}\left[0/{#2}\right]}
%\newcommand\Substpar[3]{\left({#1}\right)\left[{#2}/{#3}\right]}
\newcommand\Substpar[3]{\Bigl({#1}\Bigr)\left[{#2}/{#3}\right]}
\newcommand\Substbis[2]{{#1}[{#2}]}
\newcommand\Substapp[2]{{#1}{#2}}
\newcommand\Substlinapp[2]{{#2}[{#1}]}

\newcommand\Span[1]{\overline{#1}}
\newcommand\SN{\mathcal{N}}
\newcommand\WN{\mathcal{N}}
\newcommand\Extred[1]{\mathop{\mathrm R}^{\textrm{ext}}{(#1)}}
\newcommand\Onered[1]{\mathop{\mathrm R}^1{(#1)}}
\newcommand\NO[1]{\mathop{\mathrm N}({#1})}
\newcommand\NOD[1]{\mathop{\mathrm N_0}({#1})}



\newcommand\Freemod[2]{{#1}\left\langle{#2}\right\rangle}
\newcommand\Mofl[1]{{#1}^\#}
\newcommand\Mlext[1]{\widetilde{#1}}
\newcommand\Difflamb{\Lambda_D}
\newcommand\Terms{\Lambda_{\mathrm D}}
\newcommand\Diffmod{\Freemod R\Difflamb}

\newcommand\Factor[1]{{#1}!}
\newcommand\Binom[2]{\genfrac{(}{)}{0pt}{}{#1}{#2}}
% \newcommand\Multinom[2]{\left[#2\right]}

\newcommand\Multinom[2]{\mathsf{mn}(#2)}

\newcommand\Multinomb[2]{\genfrac{[}{]}{0pt}{}{#1}{#2}}
\newcommand\Suite[1]{\bar#1}
\newcommand\Head[1]{\mathrel{\tau^{#1}}}

\newcommand\Headlen[2]{{\mathrm{L}}({#1},{#2})}
\newcommand\Betaeq{\mathrel{\mathord\simeq_\beta}}
\newcommand\Betadeq{\mathrel{\mathord\simeq_{\beta_{\mathrm D}}}}

\newcommand\Vspace[1]{E_{#1}}
\newcommand\Real{\mathbb{R}}
%\newcommand\Realp{\mathbb{R}^+}
\newcommand\Realp{\mathbb{R}_{\geq 0}}
\newcommand\Realpnz{\mathbb{R}_{>0}}
\newcommand\Realpto[1]{(\Realp)^{#1}}
\newcommand\Realto[1]{\Real^{#1}}
\newcommand\Realptow[1]{(\Realp)^{\Web{#1}}}
\newcommand\Realpc{\overline{\Realp}}
\newcommand\Realpcto[1]{\Realpc^{#1}}
\newcommand\Izu{[0,1]}
\newcommand\Intercc[2]{[#1,#2]}
\newcommand\Interoc[2]{(#1,#2]}
\newcommand\Interco[2]{[#1,#2)}
\newcommand\Interoo[2]{(#1,#2)}
\newcommand\Rational{\mathbb Q}

\newcommand\Ring{R}
\newcommand\Linapp[2]{\left\langle{#1}\right\rangle{#2}}
\newcommand\Linappbig[2]{\Bigl\langle{#1}\Bigr\rangle{#2}}
\newcommand\Fmod[2]{{#1}\langle{#2}\rangle}
\newcommand\Fmodr[1]{{\Ring}\langle{#1}\rangle}
\newcommand\Imod[2]{{#1}\langle{#2}\rangle_\infty}
\newcommand\Imodr[1]{{\Ring}\langle{#1}\rangle_\infty}
\newcommand\Res[2]{\langle{#1},{#2}\rangle}
% \newcommand\Funofmat[1]{\widehat{#1}}
%\newcommand\Transp[1]{{}^{\mathrm{t}}\!{#1}}
\newcommand\Transp[1]{\Orth{#1}}
\newcommand\Idmat{\operatorname{I}}
\newcommand\FINMOD[1]{\operatorname{\mathbf{Fin}\,}({#1})}
\newcommand\Bcanon[1]{e_{#1}}

\newcommand\Mfin[1]{\mathcal M_\Fini({#1})}
\newcommand\Mfinc[2]{\mathcal M_{#1}({#2})}
%\newcommand\Size[1]{\Sigma({#1})}
\newcommand\Expt[2]{\operatorname{exp}_{#1}({#2})}
\newcommand\Dexpt[2]{\operatorname{exp}'_{#1}({#2})}

\newcommand\Semtype[1]{{#1}^*}
\newcommand\Semterm[2]{{#1}^*_{#2}}

\newcommand\Elem[1]{\operatorname{Elem}({#1})}
\newcommand\Fcard[1]{\operatorname{Card}({#1})}
\newcommand\Linhom[2]{\SCOTTLIN({#1},{#2})}
%\newcommand\Hom[2]{\cA({#1},{#2})}
\newcommand\Hom[2]{\operatorname{Hom}(#1,#2)}
\newcommand\Compana{\circ_\cA}

% \newcommand\Der[1]{\operatorname{\mathsf d}^{#1}}
% \newcommand\Digg[1]{\operatorname{\mathsf p}^{#1}}


%\newcommand\Conv[1]{\operatorname{c}^{#1}}
\newcommand\IConv{\mathrel{*}}
\newcommand\Exclun[1]{\operatorname{u}^{#1}}
\newcommand\Derzero[1]{\partial^{#1}_0}
\newcommand\Dermorph[1]{\partial^{#1}}
\newcommand\Dirac[1]{\delta_{#1}}
\newcommand\Diracm{\delta}

\newcommand\Lintop[1]{\lambda({#1})}
\newcommand\Neigh[2]{\operatorname{\cV}_{#1}(#2)}
\newcommand\Matrix[1]{\mathsf{M}({#1})}

\newcommand\Ev{\operatorname{\mathsf{Ev}}}
\newcommand\Evlin{\operatorname{\mathsf{ev}}}
\newcommand\REL{\operatorname{\mathbf{Rel}}}
\newcommand\RELK{\operatorname{\mathbf{Rel}_\oc}}
\newcommand\RELPOC{\operatorname{\mathbf{RelC}}}

\newcommand\Diag[1]{\Delta^{#1}}
\newcommand\Codiag[1]{\operatorname{a}^{#1}}
\newcommand\Norm[1]{\|{#1}\|}
\newcommand\Normsp[2]{\|{#1}\|_{#2}}

\newcommand\Tpower[2]{{#1}^{\otimes{#2}}}

\newcommand\Termty[3]{{#1}\vdash{#2}:{#3}}
\newcommand\Polyty[3]{{#1}\vdash_!{#2}:{#3}}

\newcommand\Ruleskip{\quad\quad\quad\quad}

\newcommand\Sterms{\Delta}
%\newcommand\Polysymb{\mathrm{p}}
\newcommand\Polysymb{!}
\newcommand\Pterms{\Delta^{\Polysymb}}
\newcommand\SPterms{\Delta^{(\Polysymb)}}
\newcommand\Nsterms{\Delta_0}
\newcommand\Npterms{\Delta_0^{\Polysymb}}
\newcommand\Nspterms{\Delta^{(\Polysymb)}_0}

\newcommand\Relspan[1]{\overline{#1}}
\newcommand\Rel[1]{\mathrel{#1}}

%\newcommand\Redone{\bar{\beta}^1_\Delta}
\newcommand\Redmult{\bar{\beta}^{\mathrm{b}}_\Delta}
\newcommand\Red{\beta_\Delta}
\newcommand\Redst[1]{\mathop{\mathsf{Red}}}

\newcommand\Redredex{\beta^1_\Delta}
\newcommand\Redredexm{\beta^{\mathrm{b}}_\Delta}


\newcommand\Multn{\mathsf{m}}
\newcommand\Shape[1]{\mathcal{T}(#1)}
\newcommand\Tay[1]{{#1}^*}

\newcommand\Deg[1]{\textsf{deg}_{#1}}
\newcommand\Linearize[2]{\mathcal L^{#1}_{#2}}
\newcommand\Fmodrel{\Fmod}

\newcommand\Redeq{=_\Delta}
\newcommand\Kriv{\mathsf K}
\newcommand\Dom[1]{\operatorname{\mathsf{D}}(#1)}
\newcommand\Cons{::}
\newcommand\Addtofun[3]{{#1}_{{#2}\mapsto{#3}}}
\newcommand\Tofclos{\mathsf T}
\newcommand\Tofstates{\mathsf T}
\newcommand\Tofstate[3]{\Tofstates(#1,#2,#3)}
\newcommand\Tofstatez[2]{\Tofstates_0(#1,#2)}
\newcommand\BT{\operatorname{\mathsf{BT}}}
\newcommand\NF{\operatorname{\mathsf{NF}}}

\newcommand\Tofst[1]{\langle#1\rangle}

\newcommand\Msubst[3]{\partial_{#3}(#1,#2)}
\newcommand\Msubstbig[3]{\partial_{#3}\bigl(#1,#2\bigr)}
\newcommand\MsubstBig[3]{\partial_{#3}\Bigl(#1,#2\Bigr)}
\newcommand\Symgrp[1]{\mathfrak S_{#1}}

\newcommand\Tcoh{\mathrel{\frownsmile}}
\newcommand\Tcohs{\mathrel{\frown}}
\newcommand\Size{\mathop{\textsf{size}}}

\newcommand\Varset{\mathcal{V}}
\newcommand\NC[1]{\langle{#1}\rangle}
\newcommand\Tuple[1]{\langle{#1}\rangle}
\newcommand\Cotuple[1]{\left[{#1}\right]}
\newcommand\Treeterms{\mathsf{T}}
\newcommand\Tree[2]{\mathop{\mathrm{tree}_{#1}}({#2})}
\newcommand\Treeeq[1]{P_{#1}}
%\newcommand\Fvar[1]{\mathcal{V}({#1})}
\newcommand\Fvar[1]{\mathop{\textsf{fv}}({#1})}
%\newcommand\Avar[1]{\mathcal{V}_A({#1})}
\newcommand\Avar[1]{\Fvar{#1}}

\newcommand\Msetofsubst[1]{\bar F}
\newcommand\Invgrp[2]{\mathsf G({#1},{#2})}
\newcommand\Invgrpsubst[3]{\mathsf G({#1},{#2},{#3})}
\newcommand\Eqofpart[1]{\mathrel{\mathord{\sim}_{#1}}}
\newcommand\Order[1]{\left|{#1}\right|}
\newcommand\Inv[1]{{#1}^{-1}}
\newcommand\Invp[1]{({#1})^{-1}}
\newcommand\Linext[1]{\widetilde{#1}}
\newcommand\Linauto{\operatorname{\mathsf{Iso}}}

%\newcommand\Card[1]{\operatorname{\mathsf{card}}(#1)}

%\newcommand\Card[1]{\Order{#1}}
\newcommand{\Ens}[1]{\{#1\}}

\newcommand\Dummy{\_}

\newcommand\Varrename[2]{{#2}^{#1}}

\newcommand\Pcoh[1]{\mathsf P{#1}}
\newcommand\Pcohp[1]{\Pcoh{(#1)}}
\newcommand\Pcohc[1]{\overline{\mathsf P}{#1}}
\newcommand\Pcohcp[1]{\Pcohc{(#1)}}
\newcommand\Pcohsig[1]{\mathsf B_1{#1}}
%\newcommand\Base[1]{e_{#1}}
%\newcommand\Base[1]{\overline{#1}}
\newcommand\Base[1]{\mathsf e_{#1}}
%\newcommand\Matapp[2]{{#1}\cdot{#2}}
\newcommand\Matapp[2]{{#1}\Compl{#2}}

\newcommand\PCOH{\mathbf{Pcoh}}
\newcommand\PCOHKL{\mathbf{Pcoh}_!}
\newcommand\PCOHEMB{\mathbf{Pcoh}_{\mathord\subseteq}}


\newcommand\Leftu{\lambda}
\newcommand\Rightu{\rho}
\newcommand\Assoc{\alpha}
\newcommand\Sym{\gamma}
\newcommand\Msetempty{\Mset{\,}}


\newcommand\Tenstg[3]{\Tens{(\Tens{#1}{#2})}{#3}}
\newcommand\Tenstd[3]{\Tens{#1}{(\Tens{#2}{#3})}}

\newcommand\Banach[1]{\mathsf e{#1}}
\newcommand\Absval[1]{\left|{#1}\right|}

\newcommand\Msetsum[1]{\Sigma{#1}}

\newcommand\Retri\zeta
\newcommand\Retrp\rho

\newcommand\Subpcs{\subseteq}
\newcommand\Cuppcs{\mathop{\cup}}

\newcommand\Impl[2]{{#1}\Rightarrow{#2}}
\newcommand\Implp[2]{({#1}\Rightarrow{#2})}
\newcommand\Basemax[1]{\mathsf c_{#1}}

\newcommand\Isosucc{\mathsf s}

\newcommand\Leqway{\ll}

\newcommand\Funofmat[1]{\mathsf{fun}(#1)}
\newcommand\Funkofmat[1]{\mathsf{Fun}(#1)}

\newcommand\Pcoin[3]{\mathsf{ran}({#1},{#2},{#3})}

% \newcommand\Tsem[2]{[{#1}]_{#2}}
% \newcommand\Tsem[1]{[{#1}]}
% \newcommand\Tseme[1]{[{#1}]^{\mathord\oc}}
% \newcommand\Psem[2]{[{#1}]_{#2}}

\newcommand\Tsem[1]{\llbracket{#1}\rrbracket}
\newcommand\Tsemrel[1]{\llbracket{#1}\rrbracket^{\REL}}
\newcommand\Tsempcoh[1]{\llbracket{#1}\rrbracket^{\PCOH}}
\newcommand\Tsemcoh[1]{\llbracket{#1}\rrbracket^{\NUCS}}
\newcommand\Tseme[1]{\llbracket{#1}\rrbracket^{\mathord\oc}}
\newcommand\Psem[2]{\llbracket{#1}\rrbracket_{#2}}
\newcommand\Psemrel[2]{\llbracket{#1}\rrbracket^{\REL}_{#2}}
\newcommand\Psemcoh[2]{\llbracket{#1}\rrbracket^{\NUCS}_{#2}}
\newcommand\Psempcoh[2]{\llbracket{#1}\rrbracket^{\PCOH}_{#2}}



\newcommand\Tnat\iota
\newcommand\Fix[1]{\operatorname{\mathsf{fix}}(#1)}
\newcommand\If[3]{\operatorname{\mathsf{if}}(#1,#2,#3)}
%\newcommand\Pred[1]{\operatorname{\mathsf{pred}}(#1)}
\newcommand\Pred[1]{\operatorname{\mathsf{pred}}(#1)}
\newcommand\Succ[1]{\operatorname{\mathsf{succ}}(#1)}
\newcommand\Num[1]{\underline{#1}}
\newcommand\Loop\Omega
\newcommand\Loopt[1]{\Omega^{#1}}
%\newcommand\Ran[3]{\operatorname{\mathsf{ran}}_{#1}(#2,#3)}
\newcommand\Ran[1]{\mathsf{ran}(#1)}
%\newcommand\Dice[1]{\operatorname{\mathsf{dice}}(#1)}
\newcommand\Dice[1]{\operatorname{\mathsf{coin}}(#1)}
\newcommand\Tseq[3]{{#1}\vdash{#2}:{#3}}
\newcommand\Ptseq[3]{{#1}\vdash_0{#2}:{#3}}
%\newcommand\Tseqst[2]{{#1}\vdash{#2}}
\newcommand\Eseq[5]{{#1}\vdash{#2}:{((#3\to #4)\to #5)}}
\newcommand\Timpl\Impl
\newcommand\Timplp\Implp
\newcommand\Simpl\Impl
\newcommand\Simplp[2]{(\Impl{#1}{#2})}

\newcommand\Pcfred{\beta_{\mathsf{cd}}}

\newcommand\PCFP{\mathsf{pPCF}}
%\newcommand\PCFD{\mathsf{dPCF}}
\newcommand\PCFD{\Lang}
\newcommand\PCF{\mathsf{PCF}}
\newcommand\PCFPZ{\mathsf{pPCF}^-}

\newcommand\Curry[1]{\operatorname{\mathsf{Cur}}({#1})}
\newcommand\Fixpcoh[1]{\operatorname{\mathsf{Fix}}_{#1}}

\newcommand\Pnat{\mathbf N}

%\newcommand\Hole{[\ ]}
%\newcommand\Holet[1]{[\ \ ]^{#1}}
%\newcommand\Hsubst[2]{{#1}[{#2}]}

\newcommand\Evcontext[1]{\mathsf C_{#1}}
\newcommand\Evhead[1]{\mathsf H_{#1}}
\newcommand\Reduct[1]{\operatorname{\mathsf{red}}({#1})}
\newcommand\Ready[1]{\operatorname{\mathsf{ready}}({#1})}
\newcommand\Undefready[1]{\operatorname{\mathsf{ready}}({#1})\mathord\uparrow}
\newcommand\Defready[1]{\operatorname{\mathsf{ready}}({#1})\mathord\downarrow}

\newcommand\Contextempty{\emptyset}

%\newcommand\States{\operatorname{\mathsf S}}

\newcommand\Stateloop[1]{\perp^{#1}}
\newcommand\Matred{\operatorname{\mathsf{Red}}}

\newcommand\Vecrow[1]{\operatorname{\mathsf r}_{#1}}
\newcommand\Veccol[1]{\operatorname{\mathsf c}_{#1}}

\newcommand\Plotkin[1]{\cR^{#1}}

\newcommand\Redone[1]{\stackrel{#1}\rightarrow}
\newcommand\Redonetr[1]{\stackrel{#1}{\rightarrow^*}}
\newcommand\Redoned{\rightarrow_{\mathsf d}}

\newcommand\Transition{\leadsto}
\newcommand\Probatransp{\operatorname{\mathsf p}}
\newcommand\Lg{\operatorname{\mathsf{lg}}}
\newcommand\Emptyseq{1}

%\newcommand\FIX[1]{\mathsf{FIX}(#1)}

\newcommand\Cbsdirect[1]{{#1}^+}
\newcommand\Cbsdual[1]{{#1}^-}
\newcommand\Cbsres[3]{\left\langle#2,#3\right\rangle_{#1}}
\newcommand\Cbsdirectn[2]{\left\|{#2}\right\|_{#1}^+}
\newcommand\Cbsdualn[2]{\left\|{#2}\right\|_{#1}^-}
\newcommand\Cbsdirectp[1]{\mathsf C_{#1}^+}
\newcommand\Cbsdualp[1]{\mathsf C_{#1}^-}

\newcommand\Cbsofpcs[1]{\mathsf{cbs}({#1})}

\newcommand\Init[2][]{\mathop{\mathord\downarrow}_{#1}{#2}}
\newcommand\Final[2][]{\mathop{\mathord\uparrow}_{#1}{#2}}
\newcommand\Poop[1]{{#1}^{\mathrm{op}}}
\newcommand\Dual[1][]{\mathrel{\mathord\perp}_{#1}}

\newcommand\PP{PP}

\newcommand\Scottsymb{\mathsf S}

% \newcommand\Weak[1]{\operatorname{\mathsf{weak}}_{#1}}
\newcommand\Weak[1]{\operatorname{\mathsf{weak}}_{#1}}
\newcommand\Contr[1]{\operatorname{\mathsf{contr}}_{#1}}
\newcommand\WeakS[1]{\Weak{#1}^\Scottsymb}
\newcommand\ContrS[1]{\Contr{#1}^\Scottsymb}

\newcommand\Contrc[1]{\operatorname{\mathsf{contr}}_{#1}}

\newcommand\Der[1]{\operatorname{\mathsf{der}}_{#1}}
%\newcommand\Coder[1]{\operatorname{\mathord\partial}_{#1}}
\newcommand\Coder{\overline{\mathsf{der}}}
\newcommand\Digg[1]{\operatorname{\mathsf{dig}}_{#1}}
\newcommand\DerS[1]{\Der{#1}^{\Scottsymb}}
\newcommand\DiggS[1]{\Digg{#1}^{\Scottsymb}}

\newcommand\Lfun{\operatorname{\mathsf{fun}}}
%\newcommand\Fun{\operatorname{\mathsf{Fun}}}
\newcommand\Fun[1]{\widehat{#1}}


\newcommand\LfunS{\Lfun^\Scottsymb}
\newcommand\FunS{\Fun^\Scottsymb}

\newcommand\Ltrace{\mathsf{tr}}
\newcommand\Trace{\mathsf{Tr}}
\newcommand\LtraceS{\mathsf{tr}^\Scottsymb}
\newcommand\TraceS{\mathsf{Tr}^\Scottsymb}

% \newcommand\Id{\operatorname{\mathsf{Id}}}
\newcommand\Id{\operatorname{\mathsf{id}}}
\newcommand\Idfun{\operatorname{\mathsf{Id}}}
\newcommand\IdS{\Id^\Scottsymb}

\newcommand\Proj[1]{\mathsf{pr}_{#1}}
\newcommand\Proje[1]{\mathsf{pr}^{\Klsymb}_{#1}}
\newcommand\ProjS[1]{\Proj{#1}^\Scottsymb}
\newcommand\EvS{\Ev^\Scottsymb}
\newcommand\EvlinS{\Evlin^\Scottsymb}

%\newcommand\Excl[1]{\IExcl{#1}}
% \newcommand\Oc[1]{\oc{#1}}
% \newcommand\Occ[1]{\oc\oc{#1}}
\newcommand\Oc{\oc}
\newcommand\Occ{\oc\oc}
\newcommand\Ocpp[1]{\oc({#1})}
%\newcommand\Int[1]{\IInt{#1}}
\newcommand\Wn[1]{\wn{#1}}
\newcommand\Wnp[1]{\wn({#1})}
%\newcommand\ExclS[1]{\oc^\Scottsymb{#1}}
%\newcommand\IntS[1]{\wn^\Scottsymb{#1}}
\newcommand\OcS{\Excl}
\newcommand\WnS{\Int}

\newcommand\Ocg{\oc_{\mathsf g}}

\newcommand\Prom[1]{#1^!}
%\newcommand\Promcm[1]{#1^!}
\newcommand\Promcm[1]{#1^+}
\newcommand\Promp[1]{(#1)^!}
\newcommand\Promm[1]{{#1}^{!!}}
\newcommand\Prommm[1]{{#1}^{!!!}}
%\newcommand\PromS[1]{{#1}^{!^\Scottsymb}}
%\newcommand\PrommS[1]{{#1}^{!^\Scottsymb!^\Scottsymb}}
\newcommand\PromS{\Prom}
\newcommand\PrommS{\Promm}

\newcommand\SCOTTLIN{\operatorname{\mathbf{ScottL}}}
\newcommand\SCOTTPOC{\operatorname{\mathbf{ScottC}}}
\newcommand\SCOTTLINKL{\operatorname{\mathbf{ScottL}}_\oc}
\newcommand\SCOTTLINK{\operatorname{\mathbf{ScottL}}_\oc}
\newcommand\PPLIN{\operatorname{\mathbf{PpL}}}
\newcommand\PPLINK{\operatorname{\mathbf{PpL}}_\oc}
\newcommand\PPPOC{\operatorname{\mathbf{PpC}}}
\newcommand\RELLIN{\operatorname{\mathbf{RelL}}}
\newcommand\PERLIN{\operatorname{\mathbf{PerL}}}
\newcommand\PERPOC{\operatorname{\mathbf{PerC}}}
\newcommand\PERLINK{\operatorname{\mathbf{PerL}_\oc}}

\newcommand\Mix{\operatorname{\mathsf{mix}}}

\newcommand\Realize[1]{\Vdash_{#1}}
\newcommand\Collapseeq[1]{\sim_{#1}}

\newcommand\Relsem[1]{\left[{#1}\right]}
%\newcommand\Perofpp[1]{\widehat{#1}}
\newcommand\Perofpp[1]{\epsilon_0({#1})}
\newcommand\Perofppf{\epsilon_0}
\newcommand\Scottofpp[1]{\sigma_0({#1})}
\newcommand\Scottofppf{\sigma_0}

\newcommand\Perofpprel[1]{\mathrel B_{#1}}
\newcommand\Perofppr[1]{\Collapseeq{\Perofpp{#1}}}
\newcommand\Perofppro[1]{\Collapseeq{\Orth{\Perofpp{#1}}}}

\newcommand\Kapp[2]{#1(#2)}

\newcommand\Left{\mathsf l}
\newcommand\Up{\mathsf u}
\newcommand\Upleft{\mathsf{ul}}
\newcommand\Upright{\mathsf{ur}}

\newcommand\Collapsecat{\operatorname{\mathsf e}}
\newcommand\Hetercat{\operatorname{\mathsf e}}
\newcommand\Hetercatmod{\operatorname{\mathsf e_{\mathsf{mod}}}}
\newcommand\Heterobjnext[1]{\ulcorner{#1}\urcorner}
\newcommand\Heterobjext[1]{\llcorner{#1}\lrcorner}
\newcommand\Heternext[1]{\ulcorner{#1}\urcorner}
\newcommand\Heterext[1]{\llcorner{#1}\lrcorner}
\newcommand\Collapseobj[1]{\ulcorner{#1}\urcorner}
\newcommand\Collapsenext{\rho}


\newcommand\EXT{\sigma}
\newcommand\COLL{\epsilon}
\newcommand\COLLL{\epsilon_0}

\newcommand\Subper{\sqsubseteq}
\newcommand\Unionper{\bigsqcup}
\newcommand\Purerel{\cD_{\mathsf r}}
\newcommand\Pureper{\cD_{\mathsf e}}
\newcommand\Pureperstep{\Phi_{\mathsf e}}

\newcommand\Subpo{\sqsubseteq}
\newcommand\Unionpo{\bigsqcup}
\newcommand\Purepo{\cD_{\mathsf s}}
\newcommand\Purepostep{\Phi_{\mathsf s}}

\newcommand\Subpp{\sqsubseteq}
\newcommand\Unionpp{\bigsqcup}
\newcommand\Purepp{\cD_{\mathsf{pp}}}
\newcommand\Pureheter{\cD_{\mathsf{h}}}
\newcommand\Pureppstep{\Phi_{\mathsf{pp}}}

\newcommand\Appmod{\operatorname{\mathsf{app}}}
\newcommand\Lammod{\operatorname{\mathsf{lam}}}

\newcommand\Kloc[1]{{#1}_{\mathord\oc}}

\newcommand\Initw[2]{\Init[\Web{#1}]{#2}}
\newcommand\Finalw[2]{\Final[\Web{#1}]{#2}}

\newcommand\Heterofpp{\mathsf h}
\newcommand\Collofper{\mathsf q}

\newcommand\Hetermod{Z}

\newcommand\Relincl\eta
\newcommand\Relrestr\rho

\newcommand\Seely{\mathsf m}
\newcommand\Seelyz{\Seely^0}
\newcommand\Seelyt{\Seely^2}
\newcommand\Monoidal{\mu}

\newcommand\Compl{\,}
\newcommand\Compv{\mathrel{\ast}}
\newcommand\Curlin{\operatorname{\mathsf{cur}}}
\newcommand\Curlininv{\Inv{\operatorname{\mathsf{cur}}}}
\newcommand\Curlinp[1]{\Curlin(#1)}
\newcommand\Cur{\operatorname{\mathsf{Cur}}}

\newcommand\Op[1]{{#1}^{\mathsf{op}}}
\newcommand\Opp[1]{(#1)^{\mathsf{op}}}
\newcommand\Kl[1]{{#1}_\oc}
\newcommand\Em[1]{{#1}^\oc}
\newcommand\Klcat[2]{{#1}_{#2}}
\newcommand\Emcat[2]{{#1}^{#2}}


\newcommand\NUM[1]{\underline{#1}}
\newcommand\SUCC{\mathsf{succ}}
\newcommand\PRED{\mathsf{pred}}
\newcommand\IF{\mathsf{if}}
\newcommand\IFV[3]{\IF(#1,(#2)\,#3)}
%\newcommand\Ifv[4]{\IF(#1,#2,(#3)\,#4)}
%\newcommand\Ifv[4]{\IF(#1,#2,[#3]\,#4)}
\newcommand\Ifv[4]{\IF(#1,#2,#3\cdot #4)}
\newcommand\FIX{\mathsf{fix}}
\newcommand\FIXV[2]{\mathsf{fix}\,#1\cdot#2}
\newcommand\FIXVT[3]{\mathsf{fix}\,#1^{#2}\,#3}
\newcommand\Fixt[3]{\mathsf{fix}\,#1^{#2}\,#3}
\newcommand\APP[2]{(#1)#2}
\newcommand\ABST[3]{\lambda #1^{#2}\, #3}
%\newcommand\MUT[3]{\mu #1:#2\, #3}
\newcommand\MUT[3]{\mu #1^{#2}\, #3}
\newcommand\MU[2]{\mu #1\, #2}
\newcommand\NAMED[2]{[#1]#2}

\newcommand\Abstpref[2]{\lambda #1^{#2}\,}

\newcommand\NAT{\iota}
\newcommand\IMPL[2]{#1\Rightarrow #2}

\newcommand\SEQ[4]{#1\vdash #2:#3\mid #4}
\newcommand\SEQI[3]{#1\vdash #2:#3}
\newcommand\SEQN[3]{#1\vdash #2\mid #3}
\newcommand\SEQP[3]{#1\vdash #2\mid #3}
\newcommand\SEQS[4]{#1\mid #2:#3\vdash #4}

\newcommand\HOLE{[\ ]}

\newcommand\Redpcf{\mathord{\to}}
\newcommand\Redpcfi{\mathord{\to_{\mathsf{PCF}}}}
\newcommand\Redclean{\relstack\to{\mathsf{cl}}}

\newcommand\Freenames{\mathsf{FN}}

\newcommand\STARG[1]{\mathsf{arg}(#1)}
\newcommand\STIF[2]{\mathsf{ifargs(#1,#2)}}
\newcommand\STSUCC{\mathsf{succ}}
\newcommand\STPRED{\mathsf{pred}}
\newcommand\EMPTY{\epsilon}
\newcommand\CONS[2]{#1\cdot #2}
\newcommand\PUSH[2]{#1\cdot #2}
\newcommand\STATE[3]{#1\star #2\mid #3}
\newcommand\TAPP[2]{#1\star#2}
\newcommand\PROC[2]{#1\star#2}

\newcommand\Div[1]{#1\uparrow}
\newcommand\Conv[2]{#1\downarrow#2}
\newcommand\Convproba[1]{\mathrel{\downarrow^{#1}}}

\newcommand\Pcftrad[1]{{#1}^\bullet}
\newcommand\Transcl[1]{{#1}^*}

\newcommand\Conn[1]{\gamma_{#1}}
\newcommand\Sing[1]{\mathsf C(#1)}
\newcommand\RELW{\operatorname{\mathbf{RelW}}}

\newcommand\Natrelw{\mathsf{N}}

\newcommand\Least{\bot}

\newcommand\Posnat{\overline{\mathsf N}}
\newcommand\Botnat{\Bot}
\newcommand\Coalgst[1]{h_{#1}}
\newcommand\Coalgca[1]{\Carrier{#1}}
% \newcommand\Coalgw[1]{\mathsf w_{#1}}
% %\newcommand\Coalgc[1]{\mathsf c_{#1}}
% \newcommand\Coalgc[1]{\mathsf k_{#1}}
\newcommand\Coalgw[1]{\mathsf{wk}_{#1}}
%\newcommand\Coalgc[1]{\mathsf c_{#1}}
\newcommand\Coalgc[1]{\mathsf{ct}_{#1}}

\newcommand\Ifrel{\mathsf{if}}

\newcommand\Eval[2]{\langle#1,#2\rangle}

%\newcommand\Let[3]{\mathsf{let}\ #1\ \mathsf{be}\ #2\ \mathsf{in}\ #3}
\newcommand\Let[3]{\mathsf{let}(#1,#2,#3)}

\newcommand\Add{\mathsf{add}}
\newcommand\Exp{\mathsf{exp}_2}
\newcommand\Cmp{\mathsf{cmp}}

\newcommand\Unift{\mathsf{unif}_2}
\newcommand\Unif{\mathsf{unif}}

\newcommand\Closed[1]{\Lambda^{#1}_0}
\newcommand\Open[2]{\Lambda^{#2}_{#1}}

\newcommand\Redmat[1]{\mathsf{Red}(#1)}
\newcommand\Redmats{\mathsf{Red}}
\newcommand\Redmato[2]{\mathsf{Red}(#1,#2)}

\newcommand\Mexpset[2]{\mathsf L(#1,#2)}

\newcommand\Expmonisoz{\Seely^0}
\newcommand\Expmonisob[2]{\Seely^2_{#1,#2}}
\newcommand\Expmonisobn{\Seely^2}

\newcommand\Injms[2]{#1\cdot#2}

\newcommand\Natobj{\mathsf{N}}
\newcommand\Natalg{h_\Natobj}

\newcommand\Snum[1]{\overline{#1}}
\newcommand\Sif{\overline{\mathsf{if}}}
\newcommand\Sifk{\overline{\mathsf{if}_{(\oc)}}}
\newcommand\Ssuc{\overline{\mathsf{suc}}}
\newcommand\Spred{\overline{\mathsf{pred}}}
\newcommand\Szero{\overline{\mathsf{zero}}}

%\newcommand\Sfix{\mathcal{Y}}
\newcommand\Sfix{\mathsf{Fix}}

\newcommand\Vect[1]{\vec{#1}}

\newcommand\Rts[1]{\cR^{#1}}

\newcommand\Probw[1]{\mathsf p(#1)}
\newcommand\Spath[2]{\mathsf{R}(#1,#2)}

\newcommand\Obseq{\sim}
\newcommand\Obsleq{\lesssim}

\newcommand\Ptest[1]{{#1}^+}
\newcommand\Ntest[1]{{#1}^-}
% \newcommand\Plen{\mathsf{len}^+}
% \newcommand\Nlen{\mathsf{len}^-}
\newcommand\Plen[1]{|#1|^+}
\newcommand\Nlen[1]{|#1|^-}

\newcommand\Shift{\mathsf{shift}}
\newcommand\Shvar[2]{\App{\Shift_{#1}}{#2}}

\newcommand\Probe{\mathsf{prob}}
\newcommand\Pprod{\mathsf{prod}}
\newcommand\Pchoose{\mathsf{choose}}

\newcommand\Argsep{\,}

\newcommand\Simplex[1]{\Delta_{#1}}

\newcommand\Embi{\eta^+}
\newcommand\Embp{\eta^-}

\newcommand\Shvec[2]{{#1}\left\{{#2}\right\}}
\newcommand\ShvecBig[2]{{#1}\Big\{{#2}\Big\}}

\newcommand\Msetu[1]{\mathsf o(#1)}
\newcommand\Msetb[2]{\mathsf o(#1,#2)}
%\newcommand\Msetb[2]{\Msetu{\{#1,#1+1,#1+#2-1\}}}

\newcommand\Mfinex[2]{\cM^-(#1,#2)}
\newcommand\Mfinr[2]{\Mfin{#1,#2}}
%\newcommand\Mfinr[2]{\Mfin{\{#1,#1+1,#1+#2-1\}}}

\newcommand\Canb[1]{\mathsf e_{#1}}

\newcommand\Prem[2]{\pi(#1,#2)}
\newcommand\Nrem[2]{\mu(#1,#2)}

\newcommand\Restrms[3]{\mathsf W(#1,#2,#3)}
\newcommand\Shleft[2]{\mathsf S(#1,#2)}

\newcommand\Listarg[3]{\,#1_{#2}\cdots#1_{#3}}

\newcommand\Rseg[2]{[#1,#2]}

\newcommand\Iftrans[2]{#1^\bullet_{#2}}

\newcommand\Bnfeq{\mathrel{\mathord:\mathord=}}
\newcommand\Bnfor{\,\,\mathord|\,\,}

\newcommand\PPCF{\mathsf{pPCF}}

\newcommand\Hempty{\ \ }
\newcommand\Hole[2]{[\Hempty]^{#1\vdash #2}}
%\newcommand\Thole[4]{#1[#2]^{#3\vdash #4}}
\newcommand\Thole[3]{#1^{#2\vdash #3}}
%\newcommand\Thsubst[4]{#1[#2]^{#3\vdash #4}}
\newcommand\Thsubst[2]{#1[#2]}

\newcommand\Tseqh[5]{\Tseq{#1}{\Thole{#2}{#3}{#4}}{#5}}

\newcommand\Locpcs[2]{{#1}_{#2}}

% dérivée pour les fonctions dans Kl(Pcoh)
\newcommand\Deriv[1]{{#1}'}

% fonction associée à un morphisme de la cat de Kl
\newcommand\Klfun[1]{\Fun{#1}}

%\newcommand\Realize{\Vdash}

\newcommand\Distsp[3]{\mathsf d_{#1}(#2,#3)}
\newcommand\Distspsymb[1]{\mathsf d_{#1}}
\newcommand\Distobs[2]{\mathsf d_{\mathsf{obs}}(#1,#2)}
\newcommand\Distobspsymb[1]{\mathsf d_{\mathsf{obs},#1}}
\newcommand\Distobsp[3]{\Distobspsymb{#1}(#2,#3)}

\newcommand\Fibloc[1]{\mathsf T#1}

\newcommand\Cuball[1]{\mathcal B#1}
\newcommand\Cuballp[1]{\mathcal B(#1)}
%\newcommand\Cuballr[2]{\mathcal B_{#1}[#2]}
\newcommand\Cuballr[2]{\Cuball{\Crel{#1}{#2}}}

% Cone local
\newcommand\Cloc[2]{{#1}_{#2}}

\newcommand\Rem[1]{\widetilde{#1}}

\newcommand\Probared[2]{\mathbb{P}(#1\downarrow #2)}

\newcommand\Tamed[2]{#1\cdot #2}

\newcommand\Mark[2]{{#1}^{#2}}

\newcommand\Oempty{\Seqempty}


\newcommand\Tone{\One}
\newcommand\Labels{\cL}

\newcommand\Onec{()}
\newcommand\Oneif[2]{#1\cdot#2}

\newcommand\Finseq[1]{{#1}^{<\omega}}

\newcommand\Ocons[2]{\Tuple{#1} #2}
\newcommand\Osingle[1]{\langle#1\rangle}
\newcommand\Ofinal[1]{\mathsf{O}(#1)}

\newcommand\Reltr[1]{\mathrel{\mathord{#1}^*}}
%\newcommand\Kminus{\overset{.} -}

\newcommand\Lpcfst{\mathsf S_\Labels}
\newcommand\Evallst{\mathsf{Ev}_\Labels}

\newcommand\Pweight[2]{\mathsf w(#1,#2)}
\newcommand\Pcompl[2]{\mathsf c(#1,#2)}
% \newcommand\Probared[2]{\mathsf P(#1\downarrow#2)}
\newcommand\Inistate[1]{\State{#1}{\Stempty}}

\newcommand\Nhead[2]{\mathsf H(#1,#2)}

%\newcommand\Expect[1]{\mathsf E(#1)}

\newcommand\Cantbopen[1]{\mathord\uparrow#1}
\newcommand\Len[1]{\mathsf{len}(#1)}

%\newcommand\PPCFlab{\PPCF_\Labels}

\newcommand\Pcfst{\mathsf S}
\newcommand\Evalst{\mathsf{Ev}}
\newcommand\Evdom[1]{\cD(#1)}

\newcommand{\Labext}{\mathsf{lab}}
\newcommand\PPCFlab{\PPCF_\Labext}
\newcommand\PCFlab{\PCF_\Labext}
\newcommand\Clabext{\mathsf{lc}}
\newcommand\PPCFlc{\PPCF_\Clabext}

\newcommand\Cantor{\cC}
\newcommand\Cantorfin{\Cantor_0}
\newcommand\Ospace{\Cantorfin}
\newcommand\Evalstlab{\Evalst_\Labext}
\newcommand\Evalstlc{\Evalst_\Clabext}
\newcommand\Evalstlcsh{\Evalst_\Clabext^\eta}
%\newcommand\Evalstlcsh{\Evalst_\Clabext^{\mathord +}}
\newcommand\Evalstlcshinv{\Evalst_\Clabext^{-\eta}}
\newcommand\Pcfstlab{\Pcfst_\Labext}
\newcommand\Pcfstlc{\Pcfst_\Clabext}
\newcommand\Striplab[1]{\underline{#1}}
\newcommand\Striplc[1]{\underline{#1}}
\newcommand\Evdomlab[1]{\cD_\Labext(#1)}
\newcommand\Evdomlc[1]{\cD_\Clabext(#1)}
\newcommand\Complstlab{\mathsf c_\Labext}

\newcommand\Dicelab[2]{\operatorname{\mathsf{lcoin}}(#1,#2)}

\newcommand\Labof[1]{\mathsf{lab}(#1)}
\newcommand\Lcof[1]{\mathsf{lc}_{#1}}

\newcommand\Pcfspy[2]{\mathsf{sp}_{#1}(#2)}

\newcommand\Evalstf[1]{\mathsf{Ev}(#1)}
\newcommand\Evalstlabf[1]{\Evalstlab(#1)}
\newcommand\Evalstlabfp[2]{\Evalstlab(#1)_{#2}}

\newcommand\Eventconvz[1]{{#1}\downarrow\Num 0}

\newcommand\Proba[1]{\mathbb P_{#1}}
\newcommand\Expect[1]{\mathbb E(#1)}

\newcommand\Spy[1]{\mathsf{sp}_{#1}}


\newcommand\Tamedc[2]{{#1}^{\langle#2\rangle}}
\newcommand\Tdistobs[3]{\mathsf d^{\langle#1\rangle}_{\mathsf{obs}}(#2,#3)}
\newcommand\Tdistobsf[1]{\mathsf d^{\langle#1\rangle}}

\newcommand\Ldistobs[2]{\mathsf d_{\mathsf{lin}}(#1,#2)}

\newcommand\Undef{\mathord\uparrow}
\newcommand\Eset[1]{\{#1\}}

\newcommand\Pneg[2]{\nu_{#1}(#2)}

\newcommand\Zeroc[1]{0_{#1}}
\newcommand\Underc[1]{\underline{#1}}
\newcommand\Sseq[4]{#1\vdash #2:#3:#4}

\newcommand\Sfun{{\mathsf S}}
\newcommand\Sfunm{\underline{\mathsf S}}
\newcommand\Sfunc{\overline{\mathsf S}}
\newcommand\Sfunb{\overline{\Sfunm}}
%\newcommand\Sfun{\bm{\mathsf{S}}}
%\newcommand\Scfun{\mathbf S_{\mathsf{can}}}
\newcommand\Scfun{\Sfun_{\Into}}
\newcommand\Sproj[1]{\operatorname\pi_{#1}}
\newcommand\Sin[1]{\operatorname{\iota}_{#1}}
%\newcommand\Ssum{\operatorname{\mathsf s}}
\newcommand\Ssum{\sigma}
\newcommand\Sflip{\operatorname{\mathsf c}}
\newcommand\Sflipl[1]{\Sflip(#1)}
\newcommand\Scflip{\widetilde{\Sflip}}
% \newcommand\Stuple[1]{\Tuple{#1}_{\Sfun}}
\newcommand\Stuple[1]{\left\llangle{#1}\right\rrangle}
\newcommand\Sctuple[1]{\Tuple{#1}_{\Scfun}}
\newcommand\Smont{\operatorname{\mathsf L}}
\newcommand\Smontz{\Smont^0}
\newcommand\Scmont{\widetilde{\Smont}}
\newcommand\Sstr{\operatorname\phi}
\newcommand\Sstrs{\Sstr^\Sym}
\newcommand\Sstrc{\Sstr^{\multimap}}
\newcommand\Sdiff{\operatorname\partial}
\newcommand\Sdiffuc{\operatorname\partial'}
\newcommand\Sdiffcaold{\delta}
\newcommand\Sdiffca{\tilde\partial}
\newcommand\Sdiffctx[2]{\Sdiff(#1,#2)}

\newcommand\Sdfun{\operatorname{\mathsf D}}
\newcommand\Sdfunc{\Sdfun_{\mathsf{cur}}} % curryfied version
\newcommand\Sdfunint{\Sdfun_{\mathsf{int}}} % curryfied version


\newcommand\Coh[1]{\coh_{#1}}
\newcommand\Scoh[1]{\scoh_{#1}}
\newcommand\Incoh[1]{\incoh_{#1}}
\newcommand\Sincoh[1]{\sincoh_{#1}}
\newcommand\Neu[1]{\equiv_{#1}}
%\newcommand\Cl[1]{\textsf{Cl}({#1})}
%\newcommand\Clfin[1]{\mbox{\textsf{Cl}}_{\mathsf{fin}}({#1})}
\newcommand\Matappa[2]{{#1}\cdot{#2}}
\newcommand\Matappap[2]{\left({#1}\cdot{#2}\right)}


\newcommand\Saxcom{(\textbf{S-com})}
\newcommand\Saxzero{(\textbf{S-zero})}
\newcommand\Saxass{(\textbf{S-assoc})}
\newcommand\Saxwit{(\textbf{S-witness})}
\newcommand\Saxdist{(\textbf{S$\ITens$-dist})}
\newcommand\Saxfun{(\textbf{S$\ITens$-fun})}
\newcommand\Saxprod{(\textbf{S$\IWith$-pres})}

\newcommand\Csaxepi{(\textbf{CS-epi})}
\newcommand\Csaxsum{(\textbf{CS-sum})}
\newcommand\Ccsaxepi{(\textbf{CCS-epi})}
\newcommand\Ccsaxsum{(\textbf{CCS-sum})}
\newcommand\Csaxflip{(\textbf{CS-flip})}

\newcommand\Sprodisoz{\mathsf p^0}
\newcommand\Sprodisot{\mathsf p^2}

\newcommand\Sone{\One}
\newcommand\Sonelem{\ast}

% \newcommand\Win[1]{\Inj{#1}^{\with}}
% \newcommand\Wdiag{\Delta^\with}
\newcommand\Win[1]{\Inj{#1}}
\newcommand\Wdiag{\Delta}
\newcommand\Into{\mathsf I}

\newcommand\Diffst{\mathsf d}
\newcommand\Obj[1]{\mathsf{Obj(#1)}}

\newcommand\Fdom{\mathsf{dom}}

\newcommand\Diffofst[1]{{#1}^{+}}
\newcommand\Diffofste[1]{{\overline{#1}}^{+}}
\newcommand\Stofdiff[1]{{#1}^{-}}

\newcommand\Sdiffst{\widetilde\partial}
\newcommand\Sdiffstcf[1]{\widetilde\partial^{#1}}

\newcommand\Diffrac[2]{\frac{d #1}{d #2}}
\newcommand\Intcc[2]{[#1,#2]}

%\newcommand\Sfunadd{\mathsf{add}}
%\newcommand\Sfunadd{\sigma}
\newcommand\Sfunadd{\tau}

\newcommand\Symbdiff[1]{\mathsf d_{#1}}

\newcommand\Forec[2]{\mathsf{rec}(#1,#2)}
\newcommand\Trec[3]{\mathsf{rec}\,(#1:#2)\,#3}

\newcommand\Tinto{\boldsymbol\Delta_\Into}

\newcommand\Adj{\mathrel{\dashv}}

\newcommand\Ftunit{\eta}
\newcommand\Ftcounit{\epsilon}

\newcommand\Daxchain{($\partial$\textbf{-chain})}
\newcommand\Daxlocal{($\partial$\textbf{-local})}
\newcommand\Daxclocal{(\textbf{C}$\partial$\textbf{-local})}
\newcommand\Daxclin{(\textbf{C}$\partial$\textbf{-lin})}
\newcommand\Daxlin{($\partial$\textbf{-lin})}
\newcommand\Daxwith{($\partial$\textbf{-}$\mathord{\IWith}$)}
\newcommand\Daxcwith{(\textbf{C}$\partial$\textbf{-}$\mathord{\IWith}$)}
\newcommand\Daxschwarz{($\partial$\textbf{-Schwarz})}
\newcommand\Daxcschwarz{(\textbf{C}$\partial$\textbf{-Schwarz})}
\newcommand\Daxcchain{(\textbf{C}$\partial$\textbf{-chain})}
\newcommand\Tysub[2]{#1 - #2}
\newcommand\Tykind[1]{\overline{#1}}
\newcommand\Typrod[3]{\Pi\,(#1:#2)#3}

\newcommand\Cseq[1]{#1\vdash}
\newcommand\Tyseq[2]{#1\vdash #2}
\newcommand\Kindofty[1]{\underline{#1}}

\newcommand\Emptycont{(\,)}
\newcommand\Treesep{\quad\quad}
\newcommand\Textsep{\hspace{6em}}

\newcommand\Sdfunit{\zeta}
\newcommand\Sdfmult{\theta}
\newcommand\Sdfstr{\psi}

\newcommand\Kllin{\mathsf{Lin}_{\mathord\oc}}

\newcommand\Tdiffsymb{\mathsf D}
\newcommand\Tdiff[1]{\Tdiffsymb{#1}}
\newcommand\Tdiffm[2]{\Tdiffsymb^{#1}{#2}}
\newcommand\Tdnat[1]{\Tdiffsymb^{#1}\Tnat}
\newcommand\Lproj[2]{\Sproj{#1}(#2)}
\newcommand\Lprojd[3]{\Sproj{#1}^{#2}(#3)}
\newcommand\Lprojs[1]{\Sproj{#1}}
\newcommand\Linj[2]{\Sin{#1}(#2)}
\newcommand\Linjd[3]{\Sin{#1}^{#2}(#3)}
\newcommand\Lin[2]{\Sin{#1}(#2)}
\newcommand\Lsum[1]{\Sdfmult(#1)}
\newcommand\Lsumd[2]{\Sdfmult^{#1}(#2)}
\newcommand\Lflip[1]{\Sflip(#1)}
\newcommand\Lflipd[2]{\Sflip^{#1}(#2)}
\newcommand\Lflipdl[3]{\Sflip^{#1}_{#2}(#3)}
\newcommand\Lflipl[2]{\Sflip_{#1}(#2)}
\newcommand\Lsums{\Sdfmult}
% \newcommand\Ldlet[3]{\text{xxxxxx}\color{red}{\partial(#1,#2,#3)}}
\newcommand\Ldlet[3]{\partial(#1,#2,#3)}
\newcommand\Ldletm[4]{\partial^{#1}(#2,#3,#4)}
\newcommand\Ldletv[2]{\partial({#1},{#2})}
%\newcommand\Ldletv[2]{{\color{red}\partial({#1},{#2})}}
\newcommand\Ldletvm[3]{\partial^{#1}({#2},{#3})}
\newcommand\Lzero{0}
\newcommand\Lzerot[1]{0^{#1}}
\newcommand\Lplus[2]{#1+#2}
\newcommand\Ldiff[1]{\Tdiff{#1}}
\newcommand\Ldapp[2]{(\Tdiff{#1}){#2}}
\newcommand\Ldappm[3]{(\Tdiffm{#1}{#2}){#3}}
\newcommand\Ldiffp[1]{\Tdiff({#1})}
\newcommand\Lfix[1]{\mathsf Y#1}
\newcommand\Llet[4]{\mathsf{let}^{#1}(#2,#3,#4)}
\newcommand\Llett[5]{\mathsf{let}_{#1}^{#2}(#3,#4,#5)}
\newcommand\Lif[4]{\mathsf{if}^{#1}(#2,#3,#4)}
\newcommand\Lift[5]{\mathsf{if}_{#1}^{#2}(#3,#4,#5)}
\newcommand\Lpred[2]{\operatorname{\mathsf{pred}}^{#1}(#2)}
\newcommand\Lsucc[2]{\operatorname{\mathsf{succ}}^{#1}(#2)}

\newcommand\Sdfunpart[2]{\Sdfun_{#1}#2}

\newcommand\Wseq[3]{#1\vdash_{w}#2:#3}

\renewcommand\Red{\to}

\newcommand\Tbundle[1]{\mathsf T#1}

\newcommand\Cpolike{Scott}

\newcommand\Mlin[1]{\widetilde{#1}}

\newcommand\Laxint{(\textbf{Int})}

\newcommand\Snatit[1]{\overline{\mathsf{it}}(#1)}

\newcommand\Slet{\overline{\mathsf{let}}}

\newcommand\Sfunpart[1]{\Sfun_{#1}}

\newcommand\Lineq{\sim_{\mathsf{lin}}}
\newcommand\Pluseq{\sim_{+}}
\newcommand\Linred{\to_{\mathsf{lin}}}
\newcommand\Topred{\to_{\mathsf{top}}}

% Evaluation contexts
\newcommand\Echole{[\ ]}
\newcommand\Ecfilled[2]{#1[#2]}

% Name of typing rules
\newcommand\Trvar{(\textbf{var})}
\newcommand\Trabs{(\textbf{abs})}
\newcommand\Trapp{(\textbf{app})}
\newcommand\Trfix{(\textbf{fix})}
\newcommand\Trnum{(\textbf{num})}
\newcommand\Trsuc{(\textbf{suc})}
\newcommand\Trpred{(\textbf{prd})}
\newcommand\Trif{(\textbf{if})}
\newcommand\Trzero{(\textbf{0})}
\newcommand\Trplsub{(+\textbf{-sub})}
\newcommand\Trprojo{(\textbf{proj1})}
\newcommand\Trprojt{(\textbf{proj2})}
\newcommand\Trprojd{(\textbf{projd})}
\newcommand\Trinj{(\textbf{inj})}
\newcommand\Trsum{(\textbf{sum})}
\newcommand\Trcirc{(\textbf{circ})}
\newcommand\Trdiff{(\textbf{diff})}
\newcommand\Trlet{(\textbf{let})}
\newcommand\Trlin{(\textbf{lin})}

\newcommand\Itrvar{(\textbf{i-var})}
\newcommand\Itrabs{(\textbf{i-abs})}
\newcommand\Itrapp{(\textbf{i-app})}
\newcommand\Itrfix{(\textbf{i-fix})}
\newcommand\Itrnum{(\textbf{i-num})}
\newcommand\Itrsuc{(\textbf{i-suc})}
\newcommand\Itrpredz{(\textbf{i-prd}$0$)}
\newcommand\Itrpredp{(\textbf{i-prd}$+$)}
\newcommand\Itrifz{(\textbf{i-if}$0$)}
\newcommand\Itrifp{(\textbf{i-if}$+$)}
\newcommand\Itrzero{(\textbf{i-0})}
\newcommand\Itrplsub{(+\textbf{i--sub})}
\newcommand\Itrproj{(\textbf{i-proj})}
\newcommand\Itradd{(\textbf{i-add})}
\newcommand\Itrprojo{(\textbf{i-proj1})}
\newcommand\Itrprojt{(\textbf{i-proj2})}
\newcommand\Itrprojd{(\textbf{i-projd})}
\newcommand\Itrinj{(\textbf{i-inj})}
\newcommand\Itrsumzz{(\textbf{i-sum}$00$)}
\newcommand\Itrsumuz{(\textbf{i-sum}$10$)}
\newcommand\Itrsumzu{(\textbf{i-sum}$01$)}
\newcommand\Itrsum{(\textbf{i-sum})}
\newcommand\Itrcirc{(\textbf{i-circ})}
\newcommand\Itrdiffz{(\textbf{i-diff}$0$)}
\newcommand\Itrdiffu{(\textbf{i-diff}$1$)}
\newcommand\Itrdiff{(\textbf{i-diff})}
\newcommand\Itrlet{(\textbf{i-let})}
\newcommand\Itrlin{(\textbf{i-lin})}



\newcommand\Iwtradd{(\textbf{i-add})}

\newcommand\Trcl[1]{#1^{\ast}}

\newcommand\Stop{\Top}

\newcommand\Tdersize[1]{\mathsf{sz}(#1)}
\newcommand\Lcht[1]{\mathsf{lh}(#1)}

\newcommand\Simplicit{sum-implicit}
\newcommand\Sharp{sharp}
\newcommand\Path{word}

% Grammar of stacks for the machine
\newcommand\Stempty{()}
\newcommand\Starg[2]{\mathsf{arg}(#1)\cdot#2}
\newcommand\Stdiff[2]{\mathsf{D}(#1)\cdot#2}
\newcommand\Stsucc[1]{\mathsf{succ}\cdot#1}
\newcommand\Stpred[1]{\mathsf{pred}\cdot#1}
\newcommand\Stif[4]{\mathsf{if}(#1,#2,#3)\cdot#4}
\newcommand\Stoneif[1]{\mathsf{seq}(#1)}
\newcommand\Stlet[4]{\mathsf{let}(#1,#2,#3)\cdot#4}
% \newcommand\State[5]{\langle#1,#2,#3,#4,#5\rangle}
% \newcommand\State[2]{\langle#1,#2\rangle}
\newcommand\Stinit[2]{\mathsf I\langle#1,#2\rangle}
\newcommand\Stfin[2]{\mathsf F\langle#1,#2\rangle}
\newcommand\Stcons{\cdot}

\newcommand\Stseq[2]{#1:#2\vdash\Tnat}
\newcommand\Tseqst[2]{#1:#2\vdash\Tnat}
\newcommand\Stseqi[4]{#1:#2:#3\vdash#4:\Tnat}
\newcommand\Etseq[1]{\vdash #1:\Tnat}
\newcommand\Etseqi[2]{\vdash #1:#2:\Tnat}

\newcommand\Stredd[1]{\to^{#1}}
\newcommand\Stred{\to}
\newcommand\Stredw{\to_{\mathsf{w}}}

\newcommand\State[3]{(#1,#2,#3)}
\newcommand\Statew[4]{(#1,#2,#3,#4)}

\newcommand\Pempty{\langle\,\rangle}

\newcommand\Stauto{$\ast$-autonomous}

\newcommand\DILL{\hbox{\textsf{DiLL}}}

\newcommand\Tonat{\Rightarrow}

\newcommand\Monz{\mu^0}
\newcommand\Mont{\mu^2}
\newcommand\Mong[1]{\mu^{#1}}

\newcommand\Tseqact[2]{#1\cdot#2}

\newcommand\Ttermi[3]{#1:#2:#3}
\newcommand\Tseqi[4]{#1\vdash\Ttermi{#2}{#3}{#4}}
\newcommand\Contca[1]{\Carrier{#1}}
\newcommand\Contz[1]{0_{#1}}

\newcommand\Itintt[2]{|#1|_{#2}}
\newcommand\Itintc[1]{\Bot(#1)}
% \newcommand\Itints[3]{\|#1\|_{#2}(#3)}
\newcommand\Itints[3]{\|#1\vdash #3\|_{#2}}
\newcommand\Itintctx[1]{|#1|}

\newcommand\Msrs[1]{\Mfin{#1}}
\newcommand\Tared{\Red_{\mathsf{top}}}

\newcommand\Rsca[1]{\underline{#1}}
\newcommand\Rsred[1]{\to_{#1}}

% \newcommand\Lang{\Lambda}
% \newcommand\States{\Theta}
\newcommand\Cdsymb{\mathsf{cd}}
% \newcommand\Lang{\Cdsymb\mathsf{PCF}}
% \newcommand\States{\Cdsymb\mathsf{KM}}
\newcommand\Lang{\PCF_\Cdsymb}
\newcommand\States{\Theta_\Cdsymb}
\newcommand\Statessi{\Theta_\Cdsymb^0}
\newcommand\Statesw{\check\Theta_\Cdsymb}
\newcommand\Strednd{\to_{\mathsf{nd}}}

\newcommand\Stctx[1]{\langle{#1}\rangle}

\newcommand\Rev[1]{\overline{#1}}

\newcommand\Rcycle[1]{\underrightarrow{#1}}
\newcommand\Lcycle[1]{\underleftarrow{#1}}

\newcommand\Itopenn[4]{|#1\vdash #2:#3|^{(#4)}}
\newcommand\Itopen[3]{|#1\vdash #2:#3|}

\newcommand\Mstrans[2]{\mathsf L(#1,#2)}
\newcommand\Mscard[1]{\##1}

\newcommand\Mspmap[2]{{#1}\ast{#2}}

\newcommand\Qforg{\mathsf Q}

\newcommand\Pchoice[3]{\mathsf{pc}^{#1}(#2,#3)}
\newcommand\Spchoice{\overline{\mathsf{pc}}}

\newcommand\Langp{\Lang^{\mathsf p}}

\newcommand\Wcell[1]{\check{#1}}
\newcommand\Intow{\check\Into}

\newcommand\Dwords[1]{\mathsf{w}(#1)}
\newcommand\Dwordl[1]{\mathsf w_0(#1)}
\newcommand\Nwcell[3]{\Sigma_{#1}(#2:#3)}

\newcommand\Wempty{\Pempty}
\newcommand\Swcell[1]{\mathsf{ws}(#1)}

\newcommand\SystF{System \textsf F}
\newcommand\LL{\hbox{\textsf{LL}}}
\newcommand\Staraut{\(\ast\)-autonomous}
\newcommand\Intlog{Intuitionistic Logic}

\newcommand\Set[1]{\{#1\}}

\newcommand\Tanspace[2]{\mathsf T_{#1}#2}
\newcommand\Tanbundle[1]{\mathsf T{#1}}

% \newcommand\CD{\textsf{CD}}
\newcommand\CD{$\Mdeg$-differentiation}

\newcommand\Dbimon[1][\cL]{\Mdeg_{#1}}
\newcommand\Dbimongen{\mathbb{D}}
\newcommand\Dbimonco{\overline\Dbimon}
\newcommand\Dbimonmo{\underline\Dbimon}
\newcommand\Dbimonbi{\underline\Dbimonco}
\newcommand\Dbimoncoalg{\widetilde{\Dbimon}}
\newcommand\Stuplet[1]{\Stuple{#1}^{\mathord\otimes}}

\newcommand\Sfunmonm{\operatorname\tau}

\newcommand\Sfunlift{\mathsf l}
\newcommand\Slift{\mathsf l}
\newcommand\Sfunstr{\phi}
\newcommand\Sfunstri{\phi^{\mathord\multimap}}

\newcommand\Dbimoncu{\Proj 0}
\newcommand\Dbimonu{\Wdiag}
\newcommand\Dbimoncm{\Wdiag}
\newcommand\Dbimonm{\overline\Sfunmonm}
\newcommand\Dbimonl{\overline\Sfunlift}

\newcommand\Klocid{\Id^{(\oc)}}

%\newcommand\Dfun{\widetilde{\mathsf D}}
\newcommand\Dfun{\mathsf T}
\newcommand\Dfunpart[1]{\Dfun_{#1}}
\newcommand\KLDFUN{\Klcat{(\Kl \cL)}{\Dfun}}

\newcommand\Derfun{\operatorname{{\mathsf{Der}}}}
\newcommand\Derfunm[1]{\mathsf{Der}_{#1}}

% \newcommand\Sfunlaxt{\widetilde\phi^2}
\newcommand\Sfunlaxt{\widetilde\phi}

\newcommand\Ddiff{\widetilde\partial}

\newcommand\ExpMon[1]{\mu^{#1}}

\newcommand\Indactms[2]{#1\cdot#2}

\newcommand\Wstren[1]{\psi^{#1}}
\newcommand\Dfunstr[1]{\Psi^{#1}}
\newcommand\Dfunstrf{\Psi^{\Rightarrow}}
%\newcommand\Swithiso{\mu^{\mathord\with}}
\newcommand\Swithiso{\widetilde\psi}
\newcommand\Dwithiso{\widetilde\Psi}

\newcommand\Dmonu{\zeta}
\newcommand\Dmonm{\theta}

\newcommand\Ap[2]{#1\left(#2\right)}
%\newcommand\A[2]{{#1}\hspace{1pt}#2}
\newcommand\A[2]{{#1}#2}

\newcommand\Dfunint{\Dfun^{\mathsf{int}}}
\newcommand\Dfunmon{\widetilde\Psi}

\newcommand\Ifd[4]{\mathsf{if}^{#1}(#2,#3,#4)}
\newcommand\Succd[2]{\mathsf{succ}^{#1}(#2)}
\newcommand\Predd[2]{\mathsf{pred}^{#1}(#2)}
\newcommand\Letd[4]{\mathsf{let}^{#1}(#2,#3,#4)}

\renewcommand\Diffsymb{\mathsf D}

\newcommand\Pd[1]{\operatorname{\Diffsymb}#1}
\newcommand\Pdinj[3]{\iota^{#1}_{#2}(#3)}
\newcommand\Pdproj[3]{\pi^{#1}_{#2}(#3)}
\newcommand\Pdinjp[3]{\iota^{#1}(#2,#3)}
\newcommand\Pdprojp[3]{\pi^{#1}(#2,#3)}
\newcommand\Pdsum[2]{\theta^{#1}(#2)}
\newcommand\Pdflip[3]{\mathsf{c}^{#1}_{#2}(#3)}

\newcommand\CDPCF{\PCF_\Diffsymb}

\newcommand\Diffm[2]{\partial(#1,#2)}

\newcommand\Extseq[1]{\langle#1\rangle}

\makeatletter
\newcommand{\dotminus}{\mathbin{\text{\@dotminus}}}

\newcommand{\@dotminus}{%
  \ooalign{\hidewidth\raise1ex\hbox{.}\hidewidth\cr$\m@th-$\cr}%
}
\makeatother

\newcommand\Kminus{\mathrel{\dotminus}}

\newcommand\Fsmod[2]{#1\langle#2\rangle}

\newcommand\Rellift[1]{{#1}^\dagger}

\newcommand\Pcfredf{\rho_{\mathsf{cd}}}
\newcommand\Coeffs{\mathbb{K}}

\newcommand\Holef[1]{[#1]}
\newcommand\Holee{\Holef\ }
\newcommand\Termofst[1]{\Stctx{#1}}

% \newcommand\Mslift[1]{\mathsf{ms}(#1)}
\newcommand\Mslift[1]{#1^\dagger}
% \newcommand\Mslifttr[1]{\mathsf{ms}(#1)^\ast}
\newcommand\Mslifttr[1]{#1^{\dagger\ast}}

\newcommand\Snatiso{\phi_\Snat}

\newcommand\Elementary{representable}
\newcommand\Elementarily{representably}

\newcommand\Degrees{I}

\newcommand\Natto{\Rightarrow}

\newcommand\Mdeg{D}
\newcommand\Mdegsl[1]{\Mdeg(#1)}
\newcommand\Mdegdom{\Mdeg^{\mathrm{dom}}}
\newcommand\Mder[1]{\bm{\partial}_{#1}}
\newcommand\Mderr[1]{\bm{\partial}^{\mathrm{rem}}_{#1}}
\newcommand\Mdiff[1]{\bm{\delta}_{#1}}
\newcommand\Mmult{\bm{\mathcal{M}}}

\newcommand\Pmon{\mathsf{P}_0}
\newcommand\Errmon{\mathsf E}
\newcommand\Errmonu{\mathsf{e}}
\newcommand\Errmonm{\mathsf{i}}
\newcommand\Seta{A}
\newcommand\Setb{B}
\newcommand\Setc{C}
\newcommand\Setd{D}
\newcommand\Err{\mathord\bot}

\newcommand\Msmon{\mathsf M_0}
\newcommand\Msimon{\mathsf M_\infty}
\newcommand\Msgmon{\mathsf M}
\newcommand\Msmonu{\mathsf u}
\newcommand\Msimonm{\Sigma}
\newcommand\Msimonu{\mathsf u}
\newcommand\Msmonm{\Sigma}
\newcommand\Natc{\overline\Nat}
\newcommand\Natcto[1]{{\overline\Nat}^{#1}}
\newcommand\Msmond{\mathsf d}
\newcommand\Errext[1]{\widetilde{#1}}

\newcommand\Pmonoid{SPCM}
\newcommand\Dpmonoid{\(\Mdeg\)-ary SPCM}
\newcommand\PMonoid{SPCM}
\newcommand\Pfmonoid{finitary SPCM}
\newcommand\PFmonoid{Finitary SPCM}
\newcommand\Pimonoid{infinitary SPCM}
\newcommand\PImonoid{Infinitary SPCM}

\newcommand\Pmenriched{SPCM-enriched}
\newcommand\Dpmenriched{\(\Mdeg\)-ary SPCM-enriched}
\newcommand\PMenriched{SPCM-enriched}
\newcommand\Pmcat{\(\Mdeg\)-ary SPCM-category}
\newcommand\Pmcats{\(\Mdeg\)-ary SPCM-categories}
\newcommand\Pmsmc{\(\Mdeg\)-ary SPCM-symmetric monoidal category}

\newcommand\Msrep[1]{\mathsf{ms}(#1)}

\newcommand\Dlift{\Slift}
\newcommand\Dsum{\Ssum}
\newcommand\Dflip{\Sflip}
% \newcommand\Lingdiffcat{linear generalized difference category}
\newcommand\Lingdiffcat{\DDIFF{} resource category}
% \newcommand\Lingrdiffcat{linear generalized representable difference category}
\newcommand\Lingrdiffcat{representable \DDIFF{} resource category}
% \newcommand\Lingrdiffcats{linear generalized representable difference categories}
% \newcommand\LIngrdiffcats{Linear generalized representable difference categories}
\newcommand\Lingrdiffcats{representable \DDIFF{} resource categories}
\newcommand\LIngrdiffcats{Representable \DDIFF{} resource categories}
\newcommand\Resid{residuated}

\newcommand\Charfun[1]{\chi_{#1}}

\newcommand\Ccmcat[1]{#1^{\mathord{\ITens}}}
\newcommand\Ccmcar[1]{\Carrier{#1}}
\newcommand\Ccmw{\mathsf w}
\newcommand\Ccmc{\mathsf c}
\newcommand\Ccmfun[1]{\Sfun[#1]}
\newcommand\Ccmfunu[1]{\zeta^{#1}}
\newcommand\Ccmfunm[1]{\tau^{#1}}
\newcommand\Ccmfundl[2]{\mathsf c^{#1,#2}}
\newcommand\Ccmproj[1]{{\mathsf p}^{\mathord{\ITens}}_{#1}}
\newcommand\Coalgproj[1]{{\mathsf p}^{\mathord{\ITens}}_{#1}}
% \newcommand\Coalgc{\mathf{c}}
% \newcommand\Coalgw{\mathf{w}}

\newcommand\Monadcat[1]{\mathbf{Mon}(#1)}
\newcommand\Comonadcat[1]{\mathbf{CoMon}(#1)}
\newcommand\Monadcar[1]{\lfloor{#1}\rfloor}
\newcommand\Monadca[1]{\Carrier{#1}}
\newcommand\Monadu[1]{\mathsf u^{#1}}
\newcommand\Monadm[1]{\mathsf m^{#1}}
\newcommand\Monadc[1]{\mathsf c^{#1}}
\newcommand\Cmonadca[1]{\Carrier{#1}}
\newcommand\Cmonadu[1]{\mathsf w^{#1}}
\newcommand\Cmonadm[1]{\mathsf k^{#1}}


\newcommand\TensL{\mathcal T}
\newcommand\TensLmon{\chi}
\newcommand\TensLmonz{\chi(0)}
\newcommand\TensLmont{\chi(2)}

% \newcommand\Sfung{\mathbf S}
\newcommand\Sfung{\mathcal H}
\newcommand\Sfungmon{\chi}
\newcommand\Sfungmonz{\Funmonoidz}
\newcommand\Sfungmont{\Funmonoidt}
\newcommand\FUN[2]{[#1,#2]}
\newcommand\DL[2]{[#1,#1]^{#2}}
\newcommand\coDL[2]{[#1,#1]^{#2 \mathsf{co}}}

\newcommand\Emforg{\mathsf{U}^{\Oc}}
\newcommand\Emfree{\mathsf{E}^{\Oc}}
\newcommand\FORG{\mathbf{U}}
\newcommand\Coalgdl[1]{\partial^{#1}}
\newcommand\Coalgdlmate[1]{\widehat\partial^{#1}}
\newcommand\Coalgdlt[1]{\widehat\partial^{#1}}

\newcommand\Klext[2]{{#1}_{#2}}
\newcommand\Emlift[2]{{#1}^{#2}}

\newcommand\CADL[1]{\mathsf{Dl}_{#1}}
\newcommand\CAcoDL[1]{\mathsf{Dl}_{#1}^{\mathsf{co}}}

\newcommand\Coalgpr[1]{\Proj{#1}^{\ITens}}
\newcommand\Coalgterm{\mathsf t^{\ITens}}

\newcommand\Ccomon[1]{{#1}^{\ITens}}
\newcommand\Ccomonca[1]{\Carrier{#1}}
\newcommand\Ccomonu[1]{\mathsf{w}^{#1}}
\newcommand\Ccomonm[1]{\mathsf{k}^{#1}}
% \newcommand\Ccomonpr[2]{\mathsf{p}^{#1}_{#2}}
\newcommand\Ccomonpr[2]{\mathsf{pr}^{\ITens}_{#2}}

\newcommand\Cmon[1]{{#1}_{\ITens}}
\newcommand\Cmonca[1]{\Carrier{#1}}
\newcommand\Cmonu[1]{\mathsf{u}^{#1}}
\newcommand\Cmonm[1]{\mathsf{m}^{#1}}
\newcommand\Cmonin[2]{\mathsf{in}^{\ITens}_{#2}}


\newcommand\Bimonadca[1]{\Carrier{#1}}
\newcommand\Bimonadm[1]{\underline{#1}}
\newcommand\Bimonadc[1]{\overline{#1}}
\newcommand\Bimonaddl[1]{\mathsf c^{#1}}

\newcommand\Monaddl{\mathsf{c}}
\newcommand\Cmonaddl{\mathsf{c}}

\newcommand\Monadsym{monad swap}
\newcommand\Cmonadsym{comonad swap}

\newcommand\Bmonca[1]{\Carrier{#1}}

\newcommand\Coalcomo{\mathsf{M}}

\newcommand\Mpunit{I}

\newcommand\Monoidca[1]{\Carrier{#1}}
\newcommand\Monoidu[1]{\mathsf u^{#1}}
\newcommand\Monoidm[1]{\mathsf m^{#1}}
\newcommand\Monoidc[1]{\mathsf c^{#1}}
\newcommand\Cmonoidca[1]{\Carrier{#1}}
\newcommand\Cmonoidu[1]{\mathsf w^{#1}}
\newcommand\Cmonoidm[1]{\mathsf k^{#1}}
\newcommand\Cmonoidc[1]{\mathsf c^{#1}}

\newcommand\Symmonoid{symmetric monoid}
\newcommand\Symmonad{symmetric monad}
\newcommand\Symcomonad{symmetric comonad}
\newcommand\Symbimonad{symmetric bimonad}
\newcommand\Symcomonoid{symmetric comonoid}
\newcommand\Symbimonoid{symmetric bimonoid}
\newcommand\SYmmonoid{Symmetric monoid}

\newcommand\Funmonoidz{\mathsf{n}^0}
\newcommand\Funmonoidt{\mathsf{n}^2}

\newcommand\Bmonoid[1]{\underline{#1}}
\newcommand\Bcmonoid[1]{\overline{#1}}

\newcommand\OSMON[1]{\mathbf{SMon}_{\ITens}(#1)}
\newcommand\OCMON[1]{\mathbf{Mon}_{\ITens}(#1)}
\newcommand\OSCMON[1]{\mathbf{SMon}^{\ITens}(#1)}
\newcommand\OCCMON[1]{\mathbf{Mon}^{\ITens}(#1)}
\newcommand\SMON[1]{\mathbf{SMon}(#1)}
\newcommand\CMON[1]{\mathbf{Mon}(#1)}
\newcommand\SCMON[1]{\mathbf{ScoMon}(#1)}
\newcommand\CCMON[1]{\mathbf{coMon}(#1)}

\newcommand\Tproj{\mathsf{pr}^{\ITens}}
\newcommand\Tinj{\mathsf{in}^{\ITens}}

\newcommand\Tuplet[1]{\Tuple{#1}^{\mathord\otimes}}
\newcommand\Cotuplet[1]{\Cotuple{#1}^{\mathord\otimes}}

\newcommand\Forgcmon{\mathsf U}
\newcommand\Freecmon{\mathsf E}
% \newcommand\Freecmonu{\epsilon^{\mathord\otimes}}
% \newcommand\Freecmoncu{\eta^{\mathord\otimes}}
\newcommand\Freecmonu{\eta^{\mathord\otimes}}
\newcommand\Freecmoncu{\epsilon^{\mathord\otimes}}

\newcommand\Tocontra{\mathrel{\overset{\circ}{\rightarrow}}}

\newcommand\Sumobj{\(\Mdeg\)-summability object}
\newcommand\SUmobj{\(Mdeg\)-summability object}

\newcommand\Cohdifflambda{coherent difference \(\lambda\)-calculus}

\newcommand\Rep[2]{\overline{#1}^{#2}}






% Monoidal functors

\newcommand\Monlaxca[1]{\Carrier{#1}}
\newcommand\Monlaxz{m^0}
\newcommand\Monlaxt{m^2}
\newcommand\Monoplaxca[1]{\Carrier{#1}}
\newcommand\Monoplaxz{n^0}
\newcommand\Monoplaxt{n^2}
\newcommand\FUNMONLAX[2]{\FUN{#1}{#2}^{\mathbf{lax}}}
\newcommand\FUNMONOPLAX[2]{\FUN{#1}{#2}^{\mathbf{oplax}}}



% Symetric monoidal category
\newcommand{\sm}{\ITens}
\newcommand{\smbis}{\bullet}
\newcommand{\smone}{1}
\newcommand{\smonebis}{I}
\newcommand{\smunitL}{\lambda^{\sm}}
\newcommand{\smunitLbis}{\lambda^{\smbis}}
\newcommand{\smunitR}{\rho^{\sm}}
\newcommand{\smunitRbis}{\rho^{\smbis}}
\newcommand{\smassoc}[1][1]{\alpha^{\sm}}
\newcommand{\smassocbis}[1][1]{\alpha^{\smbis}}
\newcommand{\smsym}{\gamma^{\sm}}
\newcommand{\smsymbis}{\gamma^{\smbis}}
\newcommand{\smtuple}{(\smcat, \sm, \smone)}
\newcommand{\smtuplebis}{(\smcatbis, \smbis, \smonebis)}
\newcommand{\smcat}{\mathcal{L}} 
\newcommand{\smcatbis}{\mathcal{L'}}

% Symetric monoidal functor
\newcommand{\smf}[1][]{F}
\newcommand{\osmfzero}[1][]{{n}^0}
\newcommand{\osmftwo}[1][]{{n}^2}
\newcommand{\osmf}[1][]{G}

% Partial monoids   
\newcommand\SPM{\mathbf{Spm}^{< \infty}}
\newcommand\SPIM{\mathbf{Spm}^{\leq \infty}}
\newcommand\SPMS{\mathbf{Spm}}
\newcommand\SPMCAT{\mathbf{SpmCat}}
\newcommand\VCAT{\cV\mathbf{Cat}}
\newcommand{\sumeq}{=}
\newcommand{\sumdef}{\downarrow}
\def\sumsub{\mathbin{\raisebox{1.3pt}{$-$}\mkern-13mu\raisebox{-1pt}{\scalebox{0.6}{$\boldsymbol{\rightarrow}$}}}}
\def\sumsubinv{\mathbin{\raisebox{1.3pt}{$-$}\mkern-13mu\raisebox{-1pt}{\scalebox{0.6}{$\boldsymbol{\leftarrow}$}}}}
\def\sumiff{\mathbin{{\raisebox{1.3pt}{$-$}\mkern-13mu\raisebox{-1pt}{\scalebox{0.6}{$\boldsymbol{\leftrightarrow}$}}}}}
\def\leqsumsub{\mathbin{\raisebox{1.2pt}{$<$}\mkern-13mu\raisebox{-2.3pt}{\scalebox{0.6}{$\boldsymbol{\rightarrow}$}}}}
\def\leqsumsubinv{\mathbin{\raisebox{1.2pt}{$<$}\mkern-13mu\raisebox{-2.3pt}{\scalebox{0.6}{$\boldsymbol{\leftarrow}$}}}}
\def\leqsumiff{\mathbin{\raisebox{1.2pt}{$<$}\mkern-13mu\raisebox{-2.3pt}{\scalebox{0.6}{$\boldsymbol{\leftrightarrow}$}}}}

% Mate isomorphism
\newcommand{\Lmate}[1][]{\lambda}
\newcommand{\Rmate}[1][]{\mu}


% Extensions and lifting

\newcommand{\Extfun}[1]{\mathbb{#1}}
\newcommand{\Liftfun}[1]{\mathbb{#1}}
\newcommand{\EXTCAT}[1]{\mathbf{Ext}_{#1}}
\newcommand{\LIFTCAT}[1]{\mathbf{Lift}_{#1}}
\newcommand{\Extforg}[1]{P_{#1}}
\newcommand{\Liftforg}[1]{P^{#1}}

% PCMS
\newcommand{\Pmuniv}{\mathsf{L}}
\newcommand{\Pimindex}{\mathcal{I}_{\leq \infty}}
\newcommand{\Pfmindex}{\mathcal{I}_{< \infty}}
\newcommand{\Pmindex}{\mathcal{I}}
% \newcommand{\Famact}[1]{#1^{\ast}}
\newcommand{\Famact}[1]{{{#1}_{\ast}}}
\newcommand{\Injection}{\hookrightarrow}
\newcommand{\Image}{\mathrm{Im}}


% Aymeric notation 

\newcommand{\CmonEmFun}{\mathsf{A}}
\newcommand{\Smashspace}[1]{\ \smashoperator{#1} \ }

\newcommand\Cohdeg[4]{\mathsf{cdeg}(#1,#2,#3,#4)}

\newcommand\Sumd{\sum{}^{(\Mdeg)}}

\newcommand\Mpositive{nonnegative}
\newcommand\Mpositivity{nonnegativity}

\newcommand\DDIFF{\(\Mdeg\)-differentiation}
\newcommand\SUMCAT{\(\Mdeg\)-summable category}
\newcommand\SUMBLE{\(\Mdeg\)-summable}
\newcommand\SUMBLTY[1][\Mdeg]{\(#1\)-summability}
\newcommand\PSUMBLTY[1][\Mdeg]{pre-\(#1\)-summability}




